Gradient Guidance for Diffusion Models: An Optimization Perspective

Diffusion models have demonstrated empirical successes in various applications and can be adapted to task-specific needs via guidance. This paper studies a form of gradient guidance for adapting a pre-trained diffusion model towards optimizing user-specified objectives. We establish a mathematical framework for guided diffusion to systematically study its optimization theory and algorithmic design. Our theoretical analysis spots a strong link between guided diffusion models and optimization: gradient-guided diffusion models are essentially sampling solutions to a regularized optimization problem, where the regularization is imposed by the pre-training data. As for guidance design, directly bringing in the gradient of an external objective function as guidance would jeopardize the structure in generated samples. We investigate a modified form of gradient guidance based on a forward prediction loss, which leverages the information in pre-trained score functions and provably preserves the latent structure. We further consider an iteratively fine-tuned version of gradient-guided diffusion where guidance and score network are both updated with newly generated samples. This process mimics a first-order optimization iteration in expectation, for which we proved O(1/K) convergence rate to the global optimum when the objective function is concave. Our code will be released at https://github.com/yukang123/GGDMOptim.git.

==> neurips/appdicies/discussion.tex <==
\section{Discussion}\label{sec:discussion}

\paragraph{Limitations} We do not see significant limitations in our analysis. The linear score class initiates the study of gradient-like guidance. We have already demonstrated that our proposed gradient guidance preserves low-dimensional structures for any score and data distribution (\cref{thm:faith_grad_guidance}). Moving forward, we aim to analyze the convergence properties for general score functions.



\paragraph{Broader Impacts} This paper's exploration of gradient-guided diffusion models offers theoretical implications that could inspire further algorithmic advancements. By establishing a connection between gradient-guided diffusion and optimization, the research opens new avenues for efficient and effective optimization through a generative approach. This work has the potential to enhance the precision and personalization of AI systems across various fields, including image synthesis and drug design. However, these techniques could also be misused to generate harmful content.


==> neurips/appdicies/posterior_dis.tex <==
\section{Generation by Backward SDE} \label{append:prof sde solution}
\DoToC


%\paragraph{Variance Control for Generated Data}
%The variance of generated samples $\{z_k\}$ directly influences their diversity.  \cref{alg:main} provides an additional feature for controlling the sample variance, by multiplying the pre-trained score function with a positive scalar $\gamma_k$. Thus $\gamma_k \cdot  s_{\theta}(x_t, t) + \texttt{G} (x_t,  t)$ is used for sampling in the backward process. $\gamma_k$ controls the variance by Lemma \ref{lmm:backward process solution}.

%\paragraph{Solution of Backward SDE}

\subsection{Posterior Distribution Characterization}
The following Lemma \ref{lmm:posterior distribution} characterizes the solution of backward SDE to which the score \eqref{equ:score with variance and guidance} is fed, the generated samples are steered by the gradient guidance $\texttt{G}_{loss}$. Note that the tuning parameter $\beta(t)$ needs to be chosen. The following lemma is derived from the perspective of conditional score to get a specified value of $\beta(t)$.

%Note that the tuning parameter
%$\beta(t)$ in \eqref{def:gradient_guidance+} is specified as
%\begin{equation}\label{equ:beta w. subspace}
%    \beta(t) = \fs{\alpha^2(t)/2}{\alpha^2(t) \sigma^2 + h(t)\dabs{ \nabla_{x_t}\rbra{g^\top \hat{\EE}[x_0|x_t]}^2}}.
%\end{equation}

%\paragraph{Choice of $\beta(t)$.} In theoretical analysis, the specification of $\beta(t)$ comes from conditional score functions of data $X = AU$, $A \in \RR^{D \times d}, U \sim \cN \rbra{\mu, I_d}$, $Y\mid X \sim \cN \rbra{g^\top X, \sigma^2}$. The score of marginal distribution $\nabla \log p_t(x_t) $ is
%\begin{equation*}
%\nabla \log p_t(x_t) = -\fs{1}{h(t)}\rbra{I_D - \alpha^2(t) A A^\top}x_t + \alpha(t) A \mu.
%\end{equation*}
%The conditional score $\nabla \log p_t(x_t \mid y)$ is
%\begin{equation*}
 %   \begin{aligned}
 %       \nabla \log p_t(x_t \mid y) &= -\fs{1}{h(t)}\rbra{I_D - \alpha^2(t) A A^\top}x_t + \alpha(t) A \mu \\
 %       &= \fs{ \alpha(t)}{ \sigma^2   + h(t)\dabs{A^\top g}^2}AA^\top g \sbra{ - \alpha(t) g^\top AA^\top x_t  + y - h(t) g^\top A \mu    }. \\
  %      %& = -  \fs{ \alpha^2(t)}{ \sigma^2   + h(t)\dabs{A^\top g}^2}AA^\top g g^\top AA^\top x_t + \fs{\alpha(t)y}{ \sigma^2 + h(t)\dabs{A^\top g}^2}AA^\top g \\&- \fs{\alpha(t) h(t)}{ \sigma^2  + h(t)\dabs{A^\top g}^2} AA^\top gg^\top A \mu.
 %   \end{aligned}
%\end{equation*}
%When selecting $\beta(t)$ as
%\begin{equation*}\label{equ:beta w. subspace groundtruth}
%    \beta(t) = \fs{\alpha^2(t)/2}{\alpha^2(t) \sigma^2 + h(t)\dabs{ \nabla_{x_t}\rbra{g^\top {\EE}[x_0|x_t]}^2}},
%\end{equation*}
%with ${\EE}[x_0|x_t] = \alpha(t) AA^\top x_t + h(t) A \mu $, it holds
%\begin{equation*}
%    \nabla \log p_t(x_t \mid y) =   \nabla \log p_t(x_t) - \beta(t) \cdot \nabla_{x_t} \rbra{y - g^\top {\EE}[x_0|x_t] }^2 =  \nabla \log p_t(x_t) + \texttt{G}_{loss}(x_t,t).
%\end{equation*}
%In other words, if we designate $\beta(t)$ as \eqref{equ:beta w. subspace groundtruth} and the pre-trained score equals with the unconditional score, then the ground truth of the conditional score equals the pre-trained score plus the designed guidance term $\texttt{G}_{loss}(x_t,t)$. Consequently, we opt for beta to be \eqref{equ:beta w. subspace}.


\begin{lemma}\label{lmm:choose beta}
    If the pre-trained score is $s_\theta(x_t,t)=- \fs{1}{h(t)}\rbra{I_D - \alpha^2(t) AA^\top }x_t + \alpha(t) A \mu $, where $A \in \RR^{D \times d}, \mu \in \RR^d $ and $\beta(t)$ is specified as
    \begin{equation}\label{equ:beta w. subspace}
        \beta(t) =  \fs{\alpha^2(t) / 2}{\alpha^2(t) \sigma^2 + h(t) \dabs{ \rbra{\nabla_{x_t}\hat{\EE}[x_0|x_t] }g  }} ,
    \end{equation}
    it holds that
    \begin{equation}\label{equ:beta_guidance_condi subspace}
    \begin{aligned}
       s_{\theta}(x_t,t) +  \texttt{G}_{loss}(x_t,t) 
      &= \rbra{ \alpha^2(t) AA^\top + h(t) I_D -  \frac{\alpha^2(t)}{\sigma^2 + g^\top AA^\top g} AA^\top g   g^\top AA^\top}^{-1}\\
      & \quad \cdot \rbra{x_t -  \alpha(t)A\mu - \alpha(t) \frac{y - g^\top A\mu}{\sigma^2 + g^\top AA^\top g} AA^\top g}
    \end{aligned}
    \end{equation}
\end{lemma}
\begin{proof}
    We first justify the formula of $s_\theta(x_t,t)$ coincides with the score function in the forward process and \eqref{equ:beta_guidance_condi subspace} coincides with the conditional score function. To be specific, suppose $X_0 = AU_0, U_0 \sim \cN \rbra{\mu, I_d}, Y = g^\top X_0 + \epsilon $ where $\epsilon \sim \cN (0, \sigma^2 I_D)$ is independent with $X_0$. In the forward process, given $X_0 = x_0$, $X_t$ can be written as $\alpha(t) x_0 + Z_t$ for $Z_t \sim \cN(0, h(t)I_D)$ independent of $x_0$. Due to the linear function assumption, we have
\begin{align*}
\begin{bmatrix}
X_t \\
Y
\end{bmatrix}
=
\begin{bmatrix}
\alpha(t)I_D & 0 & I_D \\
g^\top & 1 & 0
\end{bmatrix}
\begin{bmatrix}
x_0 \\
\epsilon \\
Z_t
\end{bmatrix}.
\end{align*}
Observing that the joint distribution of $(x_0, \epsilon, z_t)$ is Gaussian, we deduce
\begin{align*}
\begin{bmatrix}
X_t \\
Y
\end{bmatrix}
\sim \cN\left(
\begin{bmatrix}
\alpha(t) A \mu \\
g^\top A \mu
\end{bmatrix},
\begin{bmatrix}
\alpha^2(t) AA^\top + h(t) I_D & \alpha(t) AA^\top g \\
\alpha(t)g^\top AA^\top & \sigma^2 + g^\top AA^\top g
\end{bmatrix}\right).
\end{align*}
The marginal distribution of $X_t$ can be obtained as
\begin{equation*}
    X_t \sim \cN \rbra{\alpha(t) A \mu,  \alpha^2(t) AA^\top  + h(t) I_D },
\end{equation*}
and the score function for marginal distribution of $X_t$ is
\begin{equation*}
    \begin{aligned}
       \nabla \log p_t(x_t) &= - \rbra{  \alpha^2(t) AA^\top  + h(t) I_D }^{-1}\rbra{x_t - \alpha(t) A \mu } \\
       &= - \fs{1}{h(t)}\rbra{I_D - \alpha^2(t) AA^\top }\rbra{x_t - \alpha(t) A \mu }\\
       &= s_\theta(x_t,t).
    \end{aligned}
\end{equation*}
where the inverse is calculated according to Woodbury matrix identity. The conditional distribution $X_t | Y$ can be obtained as
\begin{align*}
X_t | Y \sim \cN\left(\alpha(t)A\mu + \alpha(t) \frac{y - g^\top A\mu}{\sigma^2 + g^\top AA^\top g} AA^\top g, \alpha^2(t) AA^\top + h(t) I_D -  \frac{\alpha^2(t)}{\sigma^2 + g^\top AA^\top g} AA^\top g   g^\top AA^\top \right).
\end{align*}
Thus the conditional score $\nabla \log p_t(x_t\mid y)$ is exactly \eqref{equ:beta_guidance_condi subspace}. Now we need to derive the guidance $\texttt{G}_{loss}$ computed by $s_\theta$ and $\beta(t)$ and show it satisfies \eqref{equ:beta_guidance_condi subspace}. First, we have
\begin{equation*}
    \begin{aligned}
        \hat{\EE}[x_0|x_t] = \fs{1}{\alpha(t)}\rbra{x_t + h(t) s_\theta(x_t,t)} = \alpha(t) AA^\top x_t + h(t) A \mu .
    \end{aligned}
\end{equation*}
Therefore, the guidance $\texttt{G}_{loss}$ is derived as
\begin{equation*}
    \begin{aligned}
        \texttt{G}_{loss}(x_t,t) &= 2 \beta(t) \rbra{y - g^\top \hat{\EE}[x_0|x_t]}\cdot \nabla_{x_t} \hat{\EE}[x_0|x_t] \cdot  g \\
        &= 2 \beta(t) \alpha(t) \sbra{y - \alpha(t)g^\top AA^\top x_t - h(t) g^\top A \mu}  \cdot AA^\top g.
    \end{aligned}
\end{equation*}
Now, we compare the coefficients of $x_t$, $\mu$ and $y$ in $\nabla \log p_t(x_t|y)$ and $s_\theta(x_t,t) +  \texttt{G}_{loss}(x_t,t)$. To show the two coefficients of $y$ are the same, it suffices to prove
\begin{equation}\label{equ:y coeff A}
    \rbra{ \alpha^2(t) AA^\top + h(t) I_D -  \frac{\alpha^2(t)}{\sigma^2 + g^\top AA^\top g} AA^\top g   g^\top AA^\top}^{-1} \cdot  \frac{\alpha(t)}{\sigma^2 + g^\top AA^\top g}  AA^\top g   = 2\beta(t) \alpha(t) AA^\top g.
\end{equation}
\eqref{equ:y coeff A} holds equal to
\begin{equation*}
    \begin{aligned}
    & \Leftrightarrow   \fs{1}{\sigma^2 + g^\top AA^\top g } AA^\top g = 2\beta(t) \cdot \sbra{AA^\top g  - 
     \fs{\alpha^2(t) g^\top AA^\top g  }{\sigma^2 + g^\top AA^\top g} \cdot AA^\top g} \\
     & \Leftrightarrow 1/(2\beta(t)) = \sigma^2 + h(t) g^\top AA^\top g.
    \end{aligned}
\end{equation*}
On the other hand, since $\nabla_{x_t}\hat{\EE}[x_0|x_t] = AA^\top $, we have $$\beta(t) = \fs{\alpha^2(t) / 2}{\alpha^2(t) \sigma^2 + h(t) \dabs{ \rbra{\nabla_{x_t}\hat{\EE}[x_0|x_t] }g  }} = \fs{1/2}{\sigma^2 + h(t) g^\top AA^\top g}. $$ Thus, we derive \eqref{equ:y coeff A} holds. Compare the terms regard with $\mu$, and it suffices to prove
\begin{equation*}
    \begin{aligned}
       & \quad  \rbra{ \alpha^2(t) AA^\top + h(t) I_D -  \frac{\alpha^2(t)}{\sigma^2 + g^\top AA^\top g} AA^\top g   g^\top AA^\top}^{-1} \cdot \rbra{\alpha(t)A\mu - \frac{\alpha(t)}{\sigma^2 + g^\top AA^\top g} AA^\top gg^\top A \mu  } \\
       &= \alpha(t) A \mu - 2 \beta(t) \alpha(t) h(t) AA^\top g g^\top A \mu \\
       & \Leftrightarrow  \beta(t) =    \rbra{2\rbra{\sigma^2 + g^\top AA^\top g }}^{-1}.
    \end{aligned}
\end{equation*}
Thus, we also prove the terms regard with $\mu$ are the same in $\nabla \log p_t(x_t \mid y) $ and $s_\theta(x_t,t)$. And coefficients of $x_t$ can also be derived as the same. So the proof is completed.  


\end{proof}

The following lemma characterizes the solution of backward SDE to which the score \eqref{equ:pre-train score solution subspace} is fed, the generated samples are steered by the gradient guidance $\texttt{G}_{loss}$.
\begin{lemma} \label{lmm:posterior distribution}
If the pre-trained score  $s_\theta (x_t,t)   $ is \eqref{equ:pre-train score solution subspace} and $\beta(t)$ is assigned as \eqref{equ:beta w. subspace}, substituting the score function with $s_\theta (x_t,t) + \texttt{G}_{loss}(x_t, t) $ in the backward SDE \eqref{eq:backward} yields, when $T \to \infty$,
\begin{equation*}
    X_{T}^{\leftarrow} \sim \cN\left(AA^\top \bar{x}_0 +  \frac{y - g^\top AA^\top \bar{x}_0}{\sigma^2 + g^\top AA^\top g} AA^\top g,  AA^\top  -  \frac{1}{\sigma^2 + g^\top AA^\top g} AA^\top g   g^\top AA^\top \right).
\end{equation*}
\end{lemma}

\begin{proof}
Consider $X_0 \sim \cN \rbra{A^\top \bar{x}_0, \Sigma}, Y=g^\top X_0 + \epsilon $ where $\epsilon \sim \cN \rbra{0, \sigma^2 I_D}$. Let $X_0$ be the initialization of the forward process. Denote $p_t(x_t \mid y)$ as the density of $X_t \mid Y$. According to Lemma~\ref{lmm:choose beta} and its proof (assigning $\mu = A^\top \bar{x}_0$), we get $ s_\theta (x_t,t) + \texttt{G}_{loss}(x_t, t) = \nabla \log p_t(x_t\mid y) $. Thus, the backward SDE turns out to be
\begin{equation}\label{equ:backward catch condi score}
    \diff \bXb_t = \left[\frac{1}{2} \bXb_t + \nabla \log p_{T-t}(\bXb_t\mid y)\right] \diff t + \diff \overline{W}_t, \quad \bXb_0 \sim \cN \rbra{0, I_D}.
\end{equation}
Since the initial distribution $p_0(x_0 \mid y)$ of the forward process can also be obtained by \eqref{equ:backward catch condi score} where we replace the initial distribution as $p_T(x_T\mid y)$. According to Girsanov theorem, we get the KL divergence between the terminal distribution $p_{T}^{\leftarrow} $ of \eqref{equ:backward catch condi score} and $p_0(x_0 \mid y)$.
\begin{equation*}
    \text{KL}\rbra{p_0 \mid p_{T}^{\leftarrow}  } = - \EE_{p_0} \sbra{\log \rbra{\frac{p_T}{\varphi}}},
\end{equation*}
where $p_0, p_T$ are short hands for $p_0(x_0 \mid y) $ and 
$p_T(x_T\mid y)$, and $\varphi (\cdot)$ is the density for the standard normal distribution $\cN \rbra{0, I_D}$. Since in the forward process, $p_T \to \varphi$ when $T \to \infty $, we have $\text{KL}\rbra{p_0 \mid p_{T}^{\leftarrow}  } \to 0 $ when $T \to \infty$. Thus, the proof is completed.
\end{proof}

\begin{lemma}\label{lmm:sample in subspace}
    Suppose $V \in \RR^{D \times d}$ and an estimated score has the formula $s(x_t, t) = V r(x_t, t) - \fs{1}{h(t)} \rbra{I_D - VV^\top }x_t $, where $r(\cdot,\cdot): \RR^D \times [0, \infty) \to \RR^d$, substituting the score function with $s(x_t,t)$ in the backward SDE \eqref{eq:backward} yields $X_T^{\leftarrow} \in \operatorname{Span}(V)$.

    Specifically, under Assumption~\ref{asmp:subspace_data} where data lies in $\operatorname{Span}(A)$, if $s(x_t,t) = s_\theta (x_t,t) + \texttt{G}_{loss}(x_t, t) $ where the pre-trained score $s_\theta (x_t,t)$ is \eqref{equ:pre-train score solution fully linear} and $\beta(t)$ is assigned as \eqref{equ:beta general}, then $X_T^{\leftarrow} \in \operatorname{Span}(A)$.
\end{lemma}

\begin{proof}
For the sake of convenience, we omit the superscript $\leftarrow$ of $X_t$ in the backward process. Let $X_t = X_{t,\parallel} + X_{t,\perp}$ where $X_{t,\parallel} \in \operatorname{Span}(V)$ and $X_{t,\perp} \perp \operatorname{Span}(V)$. Then, the dynamic of $X_{t,\parallel}$ and $X_{t,\perp}$ follow:
\begin{equation*}
    \dif X_{t,\parallel} = \rbra{\fs{1}{2} X_{t,\parallel} + V r(x_t,T-t)}\dif t +  VV^\top \dif \overline{W}_t,
\end{equation*}
and 
\begin{equation*}
    \dif X_{t,\perp} = \rbra{\fs{1}{2} - \fs{1}{h(T - t)} }X_{t,\perp}\dif t + (I_D - VV^\top) \dif \overline{W}_t.
\end{equation*}
$X_{t,\parallel}$ follows a linear SDE which makes solving it directly is accessible. Denote 
$$B(t) := \exp \rbra{- \int_0^t \rbra{\fs{1}{2} - \fs{1}{h(T-s)} } \dif s  }. $$ We have
\begin{equation*}
    \dif B(t)X_t = B(t) (I_D - VV^\top) \dif \overline{W}_t.
\end{equation*}
Therefore, we have
\begin{equation*}
    X_t = B(t)^{-1}X_0 + \int_0^t B(t)^{-1} B(s)(I_D - VV^\top) \dif \overline{W}_t.
\end{equation*}
The variance of $X_{t,\perp}$ can be obtained as 
\begin{equation*}
    \VV \rbra{X_{t,\perp} } = B(t)^{-2} I_D + \int_0^t B(t)^{-2} B(s)^2 \dif s \cdot (I_D - VV^\top).
\end{equation*}
And $B(t) = \fs{e^{t/2}\rbra{1 - e^{T}}}{1 - e^{-T+t}}$. Thus, we get $\VV \rbra{X_{T,\perp} }=0$ which yields $X_T^{\leftarrow} \in \operatorname{Span}(V)$. As for $s'(x_t,t) = s_\theta (x_t,t) + \texttt{G}_{loss}(x_t, t) $, it suffices to show  $ s'(x_t,t) = A r'(x_t, t) - \fs{1}{h(t)} \rbra{I_D - AA^\top }x_t $. According to Lemma \ref{lmm:posterior distribution general} and its proof, we get
\begin{equation*}
    s'(x_t,t) = - \rbra{}^{}
\end{equation*}
\begin{equation*}
    X_{T}^{\leftarrow} \sim  \cN\left(\bar{x}_0 +  \frac{y - g^\top \mu}{\sigma^2 + g^\top \bar{\Sigma}_0 g} \bar{\Sigma}_0  g,  \bar{\Sigma}_0 -  \frac{\bar{\Sigma}_0 g   g^\top \bar{\Sigma}_0}{\sigma^2 + g^\top \bar{\Sigma}_0 g}  \right).
\end{equation*}


\end{proof}






















==> neurips/appdicies/posterior_dis_Cov.tex <==
\subsection{Results for fully parameterized linear setting}
%\paragraph{Variance Control for Generated Data}
%The variance of generated samples $\{z_k\}$ directly influences their diversity.  \cref{alg:main} provides an additional feature for controlling the sample variance, by multiplying the pre-trained score function with a positive scalar $\gamma_k$. Thus $\gamma_k \cdot  s_{\theta}(x_t, t) + \texttt{G} (x_t,  t)$ is used for sampling in the backward process. $\gamma_k$ controls the variance by Lemma \ref{lmm:backward process solution}.

%\paragraph{Solution of Backward SDE}
%%%The following Lemma \ref{lmm:posterior distribution} characterizes the solution of backward SDE to which the score \eqref{equ:score with variance and guidance} is fed, the generated samples are steered by the gradient guidance $\texttt{G}_{loss}$. Note that the tuning parameter $\beta(t)$ needs to be chosen. The following lemma is derived from the perspective of conditional score to get a specified value of $\beta(t)$.

%Note that the tuning parameter
%$\beta(t)$ in \eqref{def:gradient_guidance+} is specified as
%\begin{equation}\label{equ:beta w. subspace}
%    \beta(t) = \fs{\alpha^2(t)/2}{\alpha^2(t) \sigma^2 + h(t)\dabs{ \nabla_{x_t}\rbra{g^\top \hat{\EE}[x_0|x_t]}^2}}.
%\end{equation}

%\paragraph{Choice of $\beta(t)$.} In theoretical analysis, the specification of $\beta(t)$ comes from conditional score functions of data $X = AU$, $A \in \RR^{D \times d}, U \sim \cN \rbra{\mu, I_d}$, $Y\mid X \sim \cN \rbra{g^\top X, \sigma^2}$. The score of marginal distribution $\nabla \log p_t(x_t) $ is
%\begin{equation*}
%\nabla \log p_t(x_t) = -\fs{1}{h(t)}\rbra{I_D - \alpha^2(t) A A^\top}x_t + \alpha(t) A \mu.
%\end{equation*}
%The conditional score $\nabla \log p_t(x_t \mid y)$ is
%\begin{equation*}
 %   \begin{aligned}
 %       \nabla \log p_t(x_t \mid y) &= -\fs{1}{h(t)}\rbra{I_D - \alpha^2(t) A A^\top}x_t + \alpha(t) A \mu \\
 %       &= \fs{ \alpha(t)}{ \sigma^2   + h(t)\dabs{A^\top g}^2}AA^\top g \sbra{ - \alpha(t) g^\top AA^\top x_t  + y - h(t) g^\top A \mu    }. \\
  %      %& = -  \fs{ \alpha^2(t)}{ \sigma^2   + h(t)\dabs{A^\top g}^2}AA^\top g g^\top AA^\top x_t + \fs{\alpha(t)y}{ \sigma^2 + h(t)\dabs{A^\top g}^2}AA^\top g \\&- \fs{\alpha(t) h(t)}{ \sigma^2  + h(t)\dabs{A^\top g}^2} AA^\top gg^\top A \mu.
 %   \end{aligned}
%\end{equation*}
%When selecting $\beta(t)$ as
%\begin{equation*}\label{equ:beta w. subspace groundtruth}
%    \beta(t) = \fs{\alpha^2(t)/2}{\alpha^2(t) \sigma^2 + h(t)\dabs{ \nabla_{x_t}\rbra{g^\top {\EE}[x_0|x_t]}^2}},
%\end{equation*}
%with ${\EE}[x_0|x_t] = \alpha(t) AA^\top x_t + h(t) A \mu $, it holds
%\begin{equation*}
%    \nabla \log p_t(x_t \mid y) =   \nabla \log p_t(x_t) - \beta(t) \cdot \nabla_{x_t} \rbra{y - g^\top {\EE}[x_0|x_t] }^2 =  \nabla \log p_t(x_t) + \texttt{G}_{loss}(x_t,t).
%\end{equation*}
%In other words, if we designate $\beta(t)$ as \eqref{equ:beta w. subspace groundtruth} and the pre-trained score equals with the unconditional score, then the ground truth of the conditional score equals the pre-trained score plus the designed guidance term $\texttt{G}_{loss}(x_t,t)$. Consequently, we opt for beta to be \eqref{equ:beta w. subspace}.


\begin{lemma}\label{lmm:choose beta Sigma}
    If the pre-trained score is $s_{\theta}(x_t,t) = -\rbra{\alpha^2(t) \Sigma + h(t) I_D }^{-1}\rbra{x_t - \alpha(t) \mu }$, and $\beta(t)$ is specified as
    \begin{equation}\label{equ:beta w. sigma}
        \beta(t) = \fs{1}{2} \sbra{\sigma^2 + g^\top \rbra{\Sigma^{-1} + \fs{\alpha^2(t)}{h(t)} I_D }^{-1} g     }^{-1},
    \end{equation}
    it holds that
    \begin{equation}\label{equ:beta_guidance_condi}
    \begin{aligned}
      & \quad s_{\theta}(x_t,t) +  \texttt{G}_{loss}(x_t,t) \\
      &= - \rbra{\alpha^2(t)\Sigma + h(t)I_D - \fs{\alpha^2(t)}{\sigma^2 + g^\top \Sigma g } \cdot  \Sigma g  g^\top \Sigma  }^{-1}\sbra{x_t - \rbra{ \alpha(t)\mu + \frac{\alpha(t) \rbra{y - g^\top \mu } }{\sigma^2 + g^\top \Sigma g }\cdot \Sigma g } }.
    \end{aligned}
    \end{equation}
\end{lemma}
\begin{proof}
    We first justify the formula of $s_\theta(x_t,t)$ coincides with the score function in the forward process and \eqref{equ:beta_guidance_condi} coincides with the conditional score function. To be specific, suppose $X_0 \sim \cN \rbra{\mu, \Sigma }, Y = g^\top X_0 + \epsilon $ where $\epsilon \sim \cN (0, \sigma^2 I_D)$ is independent with $X_0$. In the forward process, given $X_0 = x_0$, $X_t$ can be written as $\alpha(t) x_0 + Z_t$ for $Z_t \sim \cN(0, h(t)I_D)$ independent of $x_0$. Due to the linear function assumption, we have
\begin{align*}
\begin{bmatrix}
X_t \\
Y
\end{bmatrix}
=
\begin{bmatrix}
\alpha(t)I_D & 0 & I_D \\
g^\top & 1 & 0
\end{bmatrix}
\begin{bmatrix}
x_0 \\
\epsilon \\
Z_t
\end{bmatrix}.
\end{align*}
Observing that the joint distribution of $(x_0, \epsilon, z_t)$ is Gaussian, we deduce
\begin{align*}
\begin{bmatrix}
X_t \\
Y
\end{bmatrix}
\sim \cN\left(
\begin{bmatrix}
\alpha(t) \mu \\
g^\top \mu
\end{bmatrix},
\begin{bmatrix}
\alpha^2(t) \Sigma + h(t) I_D & \alpha(t) \Sigma g \\
\alpha(t)g^\top \Sigma & \sigma^2 + g^\top \Sigma g
\end{bmatrix}\right).
\end{align*}
The conditional distribution $X_t | Y$ can now be obtained as
\begin{align*}
X_t | Y \sim \cN\left(\alpha(t)\mu + \alpha(t) \frac{y - g^\top \mu}{\sigma^2 + g^\top \Sigma g} \Sigma  g, \alpha^2(t) \Sigma + h(t) I_D -  \frac{\alpha^2(t)}{\sigma^2 + g^\top \Sigma g} \Sigma g   g^\top \Sigma \right).
\end{align*}
Thus the conditional score $\nabla \log p_t(x_t\mid y)$ is exactly as \eqref{equ:beta_guidance_condi}. Also, the marginal distribution of $X_t$ can be obtained as
\begin{equation*}
    X_t \sim \cN \rbra{\alpha(t) \mu,  \alpha^2(t) \Sigma + h(t) I_D },
\end{equation*}
and $s_\theta(x_t,t)$ is the score function. Now we need to derive the guidance $\texttt{G}_{loss}$ computed by $s_\theta$ and $\beta(t)$ and show it satisfies \eqref{equ:beta_guidance_condi}. First, we have
\begin{equation*}
    \begin{aligned}
        \hat{\EE}[x_0|x_t] &= \fs{1}{\alpha(t)}\rbra{x_t + h(t) s_\theta(x_t,t)} \\
        &= \alpha(t) \rbra{\alpha^2(t) \Sigma + h(t) I_D }^{-1} \Sigma  x_t + {h(t)}\rbra{\alpha^2(t) \Sigma + h(t) I_D}^{-1} \mu.
    \end{aligned}
\end{equation*}
Therefore, the guidance $\texttt{G}_{loss}$ is derived as
\begin{equation*}
    \begin{aligned}
        \texttt{G}_{loss}(x_t,t) &= 2 \beta(t) \rbra{y - g^\top \hat{\EE}[x_0|x_t]}\cdot \nabla_{x_t} \hat{\EE}[x_0|x_t] \cdot  g \\
        &= 2 \beta(t) \alpha(t) \sbra{y - \alpha(t) g^\top \Sigma\rbra{\alpha^2(t) \Sigma + h(t) I_D }^{-1}   x_t + {h(t)}g^\top \rbra{\alpha^2(t) \Sigma + h(t) I_D}^{-1} \mu} \\
       & \quad  \cdot \rbra{\alpha^2(t) \Sigma + h(t) I_D }^{-1} \Sigma g.
    \end{aligned}
\end{equation*}
Now, we compare the coefficients of $x_t$, $\mu$ and $y$ in $\nabla \log p_t(x_t|y)$ and $s_\theta(x_t,t) +  \texttt{G}_{loss}(x_t,t)$. To show the two coefficients of $y$ are the same, it suffices to prove
\begin{equation}\label{equ:y coeff}
     \rbra{\alpha^2(t)\Sigma + h(t)I_D - \fs{\alpha^2(t)}{\sigma^2 + g^\top \Sigma g } \cdot  \Sigma g  g^\top \Sigma  }^{-1} \cdot \fs{\alpha(t)}{\sigma^2 + g^\top \Sigma g}\Sigma g = 2\beta(t) \alpha(t) \rbra{\alpha^2(t) \Sigma + h(t) I_D }^{-1} \Sigma g.
\end{equation}
\eqref{equ:y coeff} holds equal to
\begin{equation*}
    \begin{aligned}
    & \Leftrightarrow   \fs{1}{\sigma^2 + g^\top \Sigma g} \Sigma g = 2\beta(t) \cdot \sbra{\Sigma g  - 
     \fs{g^\top \Sigma \rbra{\alpha^2(t) \Sigma + h(t) I_D }^{-1} \Sigma g  }{\sigma^2 + g^\top \Sigma g} \cdot \Sigma g } \\
     & \Leftrightarrow 1/(2\beta(t)) = \sigma^2 + g^\top \Sigma g - g^\top \Sigma \rbra{\alpha^2(t) \Sigma + h(t) I_D }^{-1} \Sigma g.
    \end{aligned}
\end{equation*}
According to Woodbury matrix identity, we have
\begin{equation*}
    \begin{aligned}
       \rbra{\Sigma^{-1} + \fs{\alpha^2(t)}{h(t)} I_D }^{-1} = \Sigma -  \Sigma \rbra{\alpha^2(t) \Sigma + h(t) I_D }^{-1} \Sigma.
    \end{aligned}
\end{equation*}
Thus, \eqref{equ:y coeff} holds for $\beta(t)$ defined in \eqref{equ:beta w. sigma}. The coefficients of $x_t$ and $\mu$ can also be proved to be equal similarly.

\end{proof}

\begin{lemma} \label{lmm:posterior distribution Sigma}
If the pre-trained score is $s_\theta (x_t,t)   $ and $\beta(t)$ is assigned as \eqref{equ:beta w. sigma}, substituting the score function with $s_\theta (x_t,t) + \texttt{G}_{loss}(x_t, t) $ in the backward SDE \eqref{eq:backward} yields, when $T \to \infty$,
\begin{equation*}
    X_{T}^{\leftarrow} \sim  \cN\left(\alpha(t)\mu + \alpha(t) \frac{y - g^\top \mu}{\sigma^2 + g^\top \Sigma g} \Sigma  g, \alpha^2(t) \Sigma + h(t) I_D -  \frac{\alpha^2(t)}{\sigma^2 + g^\top \Sigma g} \Sigma g   g^\top \Sigma \right).
\end{equation*}
\end{lemma}

\begin{proof}
    The proof is similar to Lemma~\ref{lmm:posterior distribution}.
\end{proof}




















==> neurips/appdicies/proof_identity_cov.tex <==
\section{Omitted Proofs in \cref{sec:reg opt,sec:update pre-score}}\label{append:prof thm}
\DoToC


\subsection{Proof of Lemma \ref{lmm:simple score matching}}\label{prof:simple score matching}

\begin{proof}
Using the linear score network class $\cS$, we cast the score matching loss \eqref{equ:score match objective} into
\begin{align*}
& \quad \int_{0}^{T} \hat{\EE}_{x_0 \in \mathcal{D}} \EE_{x_t\sim\cN\rbra{\alpha(t)x_0,h(t)I_D}}  \sbra{\dabs{\nabla_{x_t} \log \phi_t(x_t|x_0)-s(x_t, t)}^2} \dif t \\
& = \int_{0}^{T} \hat{\EE}_{x_0 \in \mathcal{D}} \EE_{x_t\sim\cN\rbra{\alpha(t)x_0,h(t)I_D}}  \sbra{\dabs{-\frac{1}{h(t)} (x_t - \alpha(t)x_0) + x_t - b_t}^2} \dif t \\
& = \int_{0}^{T} \hat{\EE}_{x_0 \in \mathcal{D}} \EE_{x_t\sim\cN\rbra{\alpha(t)x_0,h(t)I_D}}  \sbra{\dabs{\left(1-\frac{1}{h(t)}\right)(x_t - \alpha(t)x_0) + (\alpha(t)x_0 - b_t)}^2} \dif t \\
& \overset{(i)}{=} \int_{0}^{T} \hat{\EE}_{x_0 \in \mathcal{D}} \left[\dabs{b_t - \alpha(t)x_0}^2\right] + \int_{0}^{T} D h(t) \left(1 - \frac{1}{h(t)}\right)^2 \dif t,
\end{align*}
where equality $(i)$ follows from computing the expectation over the conditional Gaussian distribution of $x_t | x_0$. We note that $b_t$ should minimize $\hat{\EE}_{x_0 \in \mathcal{D}} \left[\dabs{b_t - \alpha(t)x_0}^2\right]$ for any $t$, which leads to
\begin{align*}
b_t = \alpha(t) \bar{x}_0.
\end{align*}
Therefore, optimizing \eqref{equ:score match objective} over linear score network class $\cS$ gives rise to
\begin{align*}
s_\theta(x_t, t) = -x_t + \alpha(t) \bar{x}_0.
\end{align*}
\end{proof}





%For $s(x_t,t) = -x_t + b_t$,
%\begin{equation}
%\begin{aligned}
%     \dabs{\phi_t(x_t|x_0) - s(x_t,t) }^2 &= \dabs{-\fs{1}{h(t)}\rbra{x_t - \alpha(t)x_0} + x_t - b_t }^2 \\
 %    &=  \dabs{\rbra{1-\fs{1}{h(t)}}\rbra{x_t -\alpha(t)x_0 }+ \rbra{\alpha(t)x_0 - b_t} }^2.
%\end{aligned}
%\end{equation}
%The solution for \eqref{equ:score match objective} is
%\begin{equation}
%    \hat{b}_t = \alpha(t) \bar{x}_0.
%\end{equation}



\subsection{Proof of Lemma \ref{lmm:pre-trained score subspace}}\label{pf:pre-trained score subspace}
We generalize Lemma~\ref{lmm:pre-trained score subspace} to weighted score matching. Specifically, let $\{w_i\}_{i=1}^n$ be a sequence of positive weight parameters. We define weighted score matching objective function as
\begin{align}\label{eq:weighted_score_matching}
\min_{s_\theta \in \mathcal{S}} \int_{0}^{T} \sum_{i=1}^n w_i\EE_{x_t\sim\cN\rbra{\alpha(t)x_{0,i},h(t)I_D}}  \sbra{\dabs{\nabla_{x_t} \log \phi_t(x_t|x_{0,i})-s_\theta(x_t, t)}_2^2} \dif t.
\end{align}
As can be seen, $w_i$ modulates the importance of each collected samples. This weighting scheme has been adopted in practice \citep{krishnamoorthy2023diffusion}. The following result extends Lemma~\ref{lmm:pre-trained score subspace} to the weighted score matching.
\begin{lemma}\label{lmm:general weights score match}
Suppose Assumption~\ref{asmp:subspace_data} holds. Assume $\exists \cbra{x_{0,i_j}}_{j=1}^m \subseteq \cD$, $x_{0,i_j} = A u_{0,i_j}$, the empirical covariance matrix of $\cbra{u_{i_j}}_{j=1}^m$ is positive definitive. 
Let $\{w_i\}_{i=1}^n$ be a series of given positive weight parameters. Solving weighted score matching \eqref{eq:weighted_score_matching} over $\cS$ chosen as in \eqref{equ:subspace pre-train class} gives rise to
\begin{align*}
s_{\theta}(x_t,t) = %\frac{1}{h(t)} A \left(h(t)\rbra{-A^{\top} {x_t} + \alpha(t)A^\top \Bar{x}^w_0} + A^\top x_t \right)-\frac{1}{h(t)} {x_t},
AA^\top \rbra{-x_t + \alpha(t)\Bar{x}_0^{{w}}} + \frac{1}{h(t)} AA^\top x_t  -\frac{1}{h(t)} {x_t},
\end{align*}
where $\bar{x}^w_0 = \rbra{\sum_{i=1}^n w_i x_{0,i}}/\rbra{\sum_{i=1}^n w_i}$ is the weighted average.
\end{lemma}
\begin{proof}
We rewrite $s_\theta$ as
\begin{align*}
s_\theta(x_t, t) = \left(-\frac{1}{h(t)} I_D + \frac{\alpha^2(t)}{h(t)} VV^\top \right) x_t + Vb_t.
\end{align*}
Substituting $s_\theta$ into the weighted score matching loss \eqref{eq:weighted_score_matching}, we obtain
\begin{align*}
& \quad \int_{0}^{T} \sum_{i=1}^n w_i\EE_{x_t\sim\cN\rbra{\alpha(t)x_{0,i},h(t)I_D}}  \sbra{\dabs{\nabla_{x_t} \log \phi_t(x_t|x_{0,i})-s_\theta(x_t, t)}^2} \dif t \\
& = \int_{0}^{T} \sum_{i=1}^n w_i\EE_{x_t\sim\cN\rbra{\alpha(t)x_{0,i},h(t)I_D}}  \sbra{\dabs{-\frac{1}{h(t)}(x_t - \alpha(t) x_{0, i})-\rbra{-\fs{1}{h(t)}I_D + \fs{\alpha^2(t)}{h(t)}VV^\top}x_t - Vb_t }^2} \dif t \\
& = \int_{0}^{T} \sum_{i=1}^n w_i\EE_{x_t\sim\cN\rbra{\alpha(t)x_{0,i},h(t)I_D}}  \Big[\Big\lVert - \fs{\alpha^2(t)}{h(t)}VV^\top \rbra{x_t - \alpha(t) x_{0,i}} \\
& \hspace{2.5in} + \fs{1}{h(t)}\rbra{I_D - \alpha^2(t)VV^\top}\rbra{\alpha(t)x_{0,i} - Vb_t}\Big\rVert^2\Big] \dif t.
\end{align*}
Taking expectation over $x_t$ in the last display leads to
\begin{align}
& \quad \int_{0}^{T} \sum_{i=1}^n w_i\EE_{x_t\sim\cN\rbra{\alpha(t)x_{0,i},h(t)I_D}}  \sbra{\dabs{\nabla_{x_t} \log \phi_t(x_t|x_{0,i})-s_\theta(x_t, t)}^2} \dif t \nonumber \\
& = \sum_{i=1}^n w_i \left[\int_{0}^{T} \fs{\alpha^4(t)}{h^2(t)}d + \dabs{\fs{1}{h(t)}\rbra{I_D - \alpha^2(t)VV^\top}\rbra{\alpha(t)x_{0,i} - Vb_t}}^2 \dif t \right]. \label{eq:bt_minimize}
\end{align}
For any fixed time $t$ and $V$, analogous to the argument in Lemma~\ref{lmm:simple score matching}, we deduce
\begin{align*}
b_t = \alpha(t) V^\top \bar{x}^w_0
\end{align*}
is the minimizer of the \eqref{eq:bt_minimize}. Now we minimize \eqref{eq:bt_minimize} over $V$ by plugging in $b_t = \alpha(t) V^\top \bar{x}_0^w$. It holds that
\begin{align*}
& \quad \int_{0}^{T} \sum_{i=1}^n w_i\EE_{x_t\sim\cN\rbra{\alpha(t)x_{0,i},h(t)I_D}}  \sbra{\dabs{\nabla_{x_t} \log \phi_t(x_t|x_{0,i})-s_\theta(x_t, t)}^2} \dif t \\
& = \sum_{i=1}^n w_i \left[\int_{0}^{T} \fs{\alpha^4(t)}{h^2(t)}d + \dabs{\fs{1}{h(t)}\rbra{I_D - \alpha^2(t)VV^\top}\rbra{\alpha(t)x_{0,i} - \alpha(t) VV^\top \bar{x}_0^w}}^2 \dif t \right] \\
& = \sum_{i=1}^n w_i \left[\int_{0}^{T} \fs{\alpha^4(t)}{h^2(t)}d + \frac{\alpha^2(t)}{h^2(t)}\dabs{\rbra{I_D - \alpha^2(t)VV^\top}\rbra{x_{0,i} - VV^\top \bar{x}_0^w}}^2 \dif t \right] \\
& = \sum_{i=1}^n w_i \left[\int_{0}^{T} \fs{\alpha^4(t)}{h^2(t)}d + \frac{\alpha^2(t)}{h^2(t)}\dabs{\rbra{I_D - VV^\top + h(t) VV^\top}\rbra{x_{0,i} - VV^\top \bar{x}_0^w}}^2 \dif t \right].
\end{align*}
Further simplification gives rise to
\begin{align}
& \quad \int_{0}^{T} \sum_{i=1}^n w_i\EE_{x_t\sim\cN\rbra{\alpha(t)x_{0,i},h(t)I_D}}  \sbra{\dabs{\nabla_{x_t} \log \phi_t(x_t|x_{0,i})-s_\theta(x_t, t)}^2} \dif t \nonumber \\
& \overset{(i)}{=} \sum_{i=1}^n w_i \left[\int_{0}^{T} \fs{\alpha^4(t)}{h^2(t)}d + \frac{\alpha^2(t)}{h^2(t)}\dabs{\rbra{I_D - VV^\top} x_{0, i} + h(t) VV^\top \rbra{x_{0,i} - \bar{x}_0^w}}^2 \dif t \right] \nonumber \\
& = \sum_{i=1}^n w_i \left[\int_{0}^{T} \fs{\alpha^4(t)}{h^2(t)}d + \frac{\alpha^2(t)}{h^2(t)}\dabs{\rbra{I_D - VV^\top} x_{0, i}}^2 + \alpha^2(t) \dabs{VV^\top \rbra{x_{0,i} - \bar{x}_0^w}}^2 \dif t \right] \nonumber \\
& = \int_{0}^{T} \Bigg[ \fs{\alpha^4(t)}{h^2(t)}d + \frac{\alpha^2(t)}{h^2(t)}\sum_{i=1}^n \left( w_i \dabs{x_{0, i}}^2 - w_i \dabs{VV^\top x_{0, i}}^2\right) \nonumber \\
& \hspace{2in} + \alpha^2(t) \sum_{i=1}^n \left(w_i \dabs{VV^\top x_{0,i}}^2 - w_i \dabs{VV^\top \bar{x}_{0}^w}^2\right) \Bigg] \dif t \nonumber \\
& = \int_{0}^{T} \Bigg[ \fs{\alpha^4(t)}{h^2(t)}d + \frac{\alpha^2(t)}{h^2(t)}\sum_{i=1}^n w_i \left(\dabs{x_{0, i}}^2 - (h^2(t) - 1) \dabs{VV^\top x_{0, i}}^2 - h^2(t) \dabs{VV^\top \bar{x}_0^w}^2\right) \dif t  \label{eq:V_minimize} \\
& \overset{(ii)}{\geq} \int_{0}^{T} \Bigg[ \fs{\alpha^4(t)}{h^2(t)}d + \frac{\alpha^2(t)}{h^2(t)}\sum_{i=1}^n w_i \left(\dabs{x_{0, i}}^2 - (h^2(t) - 1) \dabs{ x_{0, i}}^2 - h^2(t) \dabs{ \bar{x}_0^w}^2\right) \dif t,
\label{equ:lower bound}
\end{align}
where equality $(i)$ utilizes the orthogonality between $(I_D - VV^\top)$ and $VV^\top$. We note that both $x_{0, i}$ and $\bar{x}_0^w$ are in the subspace spanned by columns of $A$, as we represent $x_{0, i}$ as $x_{0, i} = A u_{0, i}$. Accordingly, it holds that $\bar{x}_0^w = A \bar{u}_0^w$ for $\bar{u}_0^w = \frac{\sum_{i=1}^n u_{0, i} w_i}{\sum_{i=1}^n w_i}$. When $V = A$, the equality achieves in the inequality $(ii)$. Since $w_i > 0$, the coefficients of  norms $\dabs{VV^\top x_{0, i}}^2, i \in [n]$ are strictly negative. If $\hat{V}$ is a solution of \eqref{eq:weighted_score_matching}, it satisfies
\begin{equation}\label{equ:x in V}
    \hat{V}\hat{V}^\top x_{0,i} = x_{0,i}, \,\, \forall i \in [n]. 
\end{equation}
Next, we prove if \eqref{eq:weighted_score_matching} holds, $\hat{V}\hat{V}^\top = AA^\top$.
Considering $x_{0,i_j}=Au_{0,i_j}$, we have
\begin{equation*}
    \rbra{I_D - \hat{V}\hat{V}^\top } A u_{0,i_j} = A u_{0,i_j} - A u_{0,i_j} = 0.
\end{equation*}
Thus, we get
\begin{equation*}
    \rbra{I_D - \hat{V}\hat{V}^\top } A \rbra{u_{0,i_j}- \tilde{u} } = 0,
\end{equation*}
where $\tilde{u} = 1/m \sum_{j=1}^m u_{0,i_j} $. We derive
\begin{equation*}
    \begin{aligned}
        0 &= \fs{1}{m} \sum_{j=1}^m \dabs{\rbra{I_D - \hat{V}\hat{V}^\top}A\rbra{u_{0,i_j} - \tilde{u}} }_2^2 \\
        &= \text{trace}\sbra{A^\top \rbra{I_D - \hat{V}\hat{V}^\top} \rbra{I_D - \hat{V}\hat{V}^\top} A \cdot \fs{1}{n} \sum_{j=1}^m \rbra{u_{0,i_j} - \tilde{u}} \rbra{u_{0,i_j} - \tilde{u}}^\top } \\
        & \geq \nu_{\min} \text{trace}\sbra{A^\top \rbra{I_D - \hat{V}\hat{V}^\top} \rbra{I_D - \hat{V}\hat{V}^\top} A } \\
        &= \nu_{\min}  \dabs{ \rbra{I_D - \hat{V}\hat{V}^\top} A}^2_F.
    \end{aligned}
\end{equation*}
Therefore, we get
\begin{equation*}
    \rbra{I_D - \hat{V}\hat{V}^\top}A = 0,
\end{equation*}
and 
\begin{equation*}
    \rbra{I_D - \hat{V}\hat{V}^\top}AA^\top = 0.
\end{equation*}
We derive that
\begin{equation*}
    {I_D - \hat{V}\hat{V}^\top} \perp AA^\top.
\end{equation*}
We get
\begin{equation*}
    \hat{V}\hat{V}^\top = AA^\top.
\end{equation*}
Together with $\hat{b}_t = \alpha(t) \hat{V}^\top \bar{x}_0^w$, the solution of score function is
\begin{equation*}
    \begin{aligned}
        {s}_{\theta}(x_t,t) &= -\hat{V}\hat{V}^\top x_t + \hat{V}\hat{b}_t + \frac{1}{h(t)} \hat{V}\hat{V}^\top x_t  -\frac{1}{h(t)} {x_t} \\
        & =  \hat{V}\hat{V}^\top \rbra{-x_t + \alpha(t)\Bar{x}_0^{{w}}} + \frac{1}{h(t)} \hat{V}\hat{V}^\top x_t  -\frac{1}{h(t)} {x_t} \\
        &= AA^\top \rbra{-x_t + \alpha(t)\Bar{x}_0^{{w}}} + \frac{1}{h(t)} AA^\top x_t  -\frac{1}{h(t)} {x_t}.
    \end{aligned}
\end{equation*}
We complete the proof. 
\end{proof}







%To this end, we can compute
%\begin{align*}
%\sum_{i=1}^n w_i \dabs{VV^\top x_{0, i}}^2 & = {\rm Trace}\left(A^\top VV^\top A \sum_{i=1}^n w_i u_{0, i} u_{0, i}^\top \right) \quad \text{and} \\
%\sum_{i=1}^n w_i \dabs{VV^\top\bar{x}_0^w}^2 & = {\rm Trace}\left(A^\top VV^\top A \sum_{i=1}^n w_{i} \bar{u}_0^w (\bar{u}_0^w)^\top \right).
%\end{align*}
%Consider an SVD of $\sum_{i=1}^n w_i u_{0, i}u_{0, i}^\top = Q\Sigma Q^\top$, where $\Sigma$ is diagonal and full rank by Assumption~\ref{asmp:data rank}. 
%\end{proof}
%We restate the lemma as
%\begin{lemma}\label{lmm:gen_pretrain solution}
%For training data $\cD = \cbra{x_{0,i}}_{i=1}^n$ and weights $\cbra{w_i}_{i=1}^n$, under Assumption \ref{asmp:subspace_data} that $x_{0,i} \in \operatorname{Span}(A)$, we opt for function class \eqref{equ:subspace pre-train class} to solve the score matching objective
%\begin{equation}\label{equ:weight score match obj}
%    \min_{s\in \mathcal{S}} \int_{0}^{T} \sum_{i=1}^n w_i\EE_{x_t\sim\cN\rbra{\alpha(t)x_{0,i},h(t)}}  \sbra{\dabs{\nabla_{x_t} \log \phi_t(x_t|x_{0,i})-s(x_t, t)}_2^2} \dif t.
%\end{equation}
%The solution is 
%\begin{equation}
%    s_{\theta}(x_t,t) = AA^\top \rbra{-x_t + \alpha(t)\Bar{x}} + \frac{1}{h(t)} AA^\top x_t  -\frac{1}{h(t)} {x_t},,
%\end{equation}
%where $\bar{x} = \rbra{\sum_{i=1}^n w_i x_{0,i}}/\rbra{\sum_{i=1}^n w_i}$.
%\end{lemma}

%\begin{proof}
 %   Rearrange the score as expression:
 %   \begin{equation}
 %      s(x_t,t) =  \rbra{-\fs{1}{h(t)} + \fs{\alpha^2(t)}{h(t)}VV^\top}x_t + Vb_t.
 %   \end{equation}
%We have $\phi_t(x_t\mid x_{0,i}) = - \fs{1}{h(t)}\rbra{x_t - \alpha(t) x_{0,i}}$. Thus
%\begin{equation}
%    \begin{aligned}
 %       \phi_t(x_t\mid x_{0,i}) - s(x_t,t) &= - \fs{1}{h(t)}\rbra{x_t - \alpha(t) x_{0,i}} - \rbra{\rbra{-\fs{1}{h(t)} + \fs{\alpha^2(t)}{h(t)}VV^\top}x_t + Vb_t} \\
  %      &= - \fs{\alpha^2(t)}{h(t)}VV^\top \rbra{x_t - \alpha(t) x_{0,i}} + \fs{1}{h(t)}\rbra{I - \alpha^2(t)VV^\top}\rbra{\alpha(t)x_{0,i} - Vb_t}.
  %  \end{aligned}
%\end{equation}
%Therefore, taking the expectation over $x_t \sim \cN\rbra{\alpha(t)x_{0,i},h(t)} $, we get
%\begin{equation}
%    \begin{aligned}
 %       \ell(x_{0,i},t) & := \EE_{x_t \sim \cN\rbra{\alpha(t)x_{0,i},h(t)}} \dabs{\phi_t(x_t\mid x_{0,i}) - s(x_t,t)}^2 \\
  %      &= \EE_{x_t \sim \cN\rbra{\alpha(t)x_{0,i},h(t)}} \dabs{- \fs{\alpha^2(t)}{h(t)}VV^\top \rbra{x_t - \alpha(t) x_{0,i}} }^2  + \dabs{\fs{1}{h(t)}\rbra{I - \alpha^2(t)VV^\top}\rbra{\alpha(t)x_{0,i} - Vb_t}}^2 \\
   %     &= \fs{\alpha^4(t)}{h^2(t)}d + \dabs{\fs{1}{h(t)}\rbra{I - \alpha^2(t)VV^\top}\rbra{\alpha(t)x_{0,i} - Vb_t}}^2.
   % \end{aligned}
%\end{equation}
%Thus,
%\begin{equation}
%    \begin{aligned}
%        \fs{\partial \ell(x_{0,i},t) }{\partial b_t} &= \fs{1}{h^2(t)}V^\top\rbra{I - \alpha^2(t)VV^\top}^2 \rbra{Vb_t - \alpha(t) x_{0,i}} \\
 %       &= b_t - \alpha(t)Vx_{0,i}. 
 %   \end{aligned}
%\end{equation}
%It results the solution for $b_t$:
%\begin{equation}
%    \hat{b}_t = \alpha(t)V \bar{x},
%\end{equation}
%where
%\begin{equation}
%    \bar{x} = \fs{\sum_{i=1}^n w_i x_{0,i}}{\sum_{i=1}^n w_i}. 
%\end{equation}

%Substitute $\hat{b}_t$ in $\ell(x_{0,i},t)$, we get
%\begin{equation}
%    \begin{aligned}
 %       \ell(x_{0,i},t) &= \fs{\alpha^4(t)}{h^2(t)}d + \dabs{\fs{\alpha(t)}{h(t)} \rbra{I-VV^\top}x_{0,i}}^2 + \dabs{\alpha(t)VV^\top\rbra{x_{0,i}-\bar{x}}}^2 \\
  %      &= \fs{\alpha^4(t)}{h^2(t)}d + \fs{\alpha^2(t)}{h^2(t)}\rbra{\dabs{x_{0,i}}^2 - \dabs{VV^\top x_{0,i}}^2 } + \alpha^2(t) \dabs{VV^\top\rbra{x_{0,i}-\bar{x}}}^2.
   % \end{aligned}
%\end{equation}
%Therefore,
%\begin{equation}
%    \begin{aligned}
 %       \sum_{i=1}^n w_i \ell(x_{0,i},t) = -\alpha^2(t)\rbra{\fs{1}{h^2(t)}-1}\rbra{\sum_{i=1}^n w_i \dabs{VV^\top x_{0,i} }^2} - \alpha^2(t) \rbra{\sum_{i=1}^n w_i } \dabs{VV^\top \bar{x}}^2 + C.
  %  \end{aligned}
%\end{equation}


%For any $V \in \RR^{D \times d}$ with orthogonal columns, it holds
%\begin{equation}\label{equ:proj norm inequ}
%    \begin{aligned}
 %       \dabs{VV^\top x_{0,i} }^2 &\leq \dabs{x_{0,i}}^2 \\
  %       \dabs{VV^\top \bar{x} }^2 &\leq \dabs{\bar{x}}^2.
  %  \end{aligned}
%\end{equation}

%Since $x_{0,i} \in \operatorname{Span}(A)$, then $\bar{x} \in \operatorname{Span}(A)$, the equality achieves in \eqref{equ:proj norm inequ} when $V = A$. Therefore, $V$ is the solution of objective \eqref{equ:score match objective} if and only if
%\begin{equation}\label{equ:x in V}
 %   VV^\top x_{0,i} = x_{0,i}, \,\, \forall i \in [n]. 
%\end{equation}

%Now we prove if \eqref{equ:x in V} holds, $VV^\top = AA^\top$.

%With $x_{0,i} = A u_{0,i}$, 
%\begin{equation*}
%    \rbra{I_D - VV^\top}Au_{0,i} = Au_{0,i} - Au_{0,i} = 0.
%\end{equation*}
%Thus,
%\begin{equation*}
%    \rbra{I_D - VV^\top}A\rbra{u_{0,i} - \bar{u}} = 0,
%\end{equation*}
%where $\bar{u} = \fs{1}{n} \sum_{i=1}^n u_{0,i}$. 

%We have
%\begin{equation*}
 %   \begin{aligned}
  %      0 &= \fs{1}{n} \sum_{i=1}^n \dabs{\rbra{I_D - VV^\top}A\rbra{u_{0,i} - \bar{u}} }_2^2 \\
  %      &= \text{trace}\sbra{A^\top \rbra{I_D - VV^\top} \rbra{I_D - VV^\top} A \cdot \fs{1}{n} \sum_{i=1}^n \rbra{u_{0,i} - \bar{u}} \rbra{u_{0,i} - \bar{u}}^\top } \\
   %     & \geq \nu_{\min} \text{trace}\sbra{A^\top \rbra{I_D - VV^\top} \rbra{I_D - VV^\top} A } \\
    %    &= \nu_{\min}  \dabs{\rbra{I_D - VV^\top} A}^2_F.
    %\end{aligned}
%\end{equation*}

%Therefore, 
%\begin{equation*}
 %   \rbra{I_D - VV^\top} A =  0.
%\end{equation*}

    
%\end{proof}







%\hui{Adapt to projected gradient ascent}
%\begin{proof}
%    Since $f$ is convex and $\lambda$-smooth, $h(x) = f(x)  - \lambda / 2 \dabs{x - \Bar X_0}^2$ is concave and $\lambda$-smooth. Due to the smoothness,
%    \begin{equation}
 %       h(z_{k+1}) \geq h(z_k) + \nabla h(z_k)^\top (z_{k+1} - z_k) - \fs{\lambda}{2} \dabs{z_{k+1}- z_k}^2.
 %   \end{equation}
 %   According to the concavity,
 %   \begin{equation}
 %       h(z_k) \geq h(x^\star) + \nabla h(z_k)^\top (z_k - x^\star).   \end{equation}
  %  Thus,
  %  \begin{equation}
  %       h(z_{k+1}) - h(x^\star) \leq \nabla h(z_k)^\top (x^\star - z_{k+1}) + \fs{\lambda}{2} \dabs{z_{k+1}- z_k}^2.
 %   \end{equation}
 %Take the expectation,
    %\begin{equation}
        %\begin{aligned}
             %\EE [ h(z_{k+1}) - h(x^\star)] &\leq \EE %\sbra{ \fs{1}{\eta}  (z_{k+1} - z_k)%(x^\star - z_{k+1}) }+ \lambda %\text{trace}\rbra{\VV (z_{k+1})} + \EE %\fs{\lambda}{2} \dabs{z_{k+1}- z_k}^2 \\
             %&=   \EE  \sbra{\fs{\lambda}{2} %\dabs{x^\star - z_k}^2 - \dabs{x^\star - %z_{k+1}}^2} +\lambda \gamma_k^2 \rbra{d - %\fs{\dabs{\nabla f(z_k)}^2}{\sigma^2_k / %\gamma^2_k + \dabs{\nabla f(z_k)}^2}}\\
             %&\leq \EE  \sbra{\fs{\lambda}{2} %\dabs{x^\star - z_k}^2 - \dabs{x^\star - %z_{k+1}}^2} + \lambda \gamma_k^2 d.
  %      \end{aligned}
 %   \end{equation}
%\end{proof}



















%\subsection{Proof of \cref{lmm:simple score matching subspace}}\label{prof:simple score matching subspace}



%\begin{proof}
%    For $s(x_t,t) = - V \rbra{V^\top x_t - b_t} - \fs{1}{h(t)} \rbra{I_D - VV^\top} x_t $,
%\begin{equation}
 %   \begin{aligned}
 %       \dabs{\phi_t(x_t|x_0) - s(x_t,t) }^2 &= \dabs{-\fs{1}{h(t)}\rbra{x_t - \alpha(t) x_0 }  + V \rbra{V^\top x_t - b_t} + \fs{1}{h(t)} \rbra{I_D - VV^\top} x_t     }^2  \\
  %      &= \dabs{ -\fs{\alpha^2(t)}{h(t)}VV^\top \rbra{x_t - \alpha(t)x_t} + \rbra{\fs{I-VV^\top}{h(t)} + VV^\top   } \rbra{\alpha(t)x_0 - V b_t}   }^2,
   % \end{aligned}
%\end{equation}

%thus,

%\begin{equation}\label{equ:score mid}
 %   \begin{aligned}
  %      &\quad \EE_{x_t\sim \cN \rbra{\alpha(t)x_0, h(t)I_D}} \dabs{\phi_t(x_t|x_0) - s(x_t,t) }^2 \\
   %     &= \EE_{x_t\sim \cN \rbra{\alpha(t)x_0, h(t)I_D}}\sbra{ \dabs{ -\fs{\alpha^2(t)}{h(t)}VV^\top \rbra{x_t - \alpha(t)x_t}}^2 + \dabs{ \rbra{\fs{I-VV^\top}{h(t)} + VV^\top   } \rbra{\alpha(t)x_0 - V b_t}   }^2 } \\
     %   &= \fs{\alpha^4(t)}{h(t)}\text{trace}(VV^\top)  + \dabs{ \rbra{\fs{I-VV^\top}{h(t)} + VV^\top   } \rbra{\alpha(t)x_0 - V b_t}   }^2. 
    %\end{aligned}
%\end{equation}

%Therefore, for a estimate $\hat{V}$ for $V$, solving \eqref{equ:score match objective} for $b_t$, 
%\begin{equation}
%    \min \hat{\EE}_{x_0 \sim \cD } \dabs{ \rbra{\fs{I-\hat{V}\hat{V}^\top}{h(t)} + \hat{V}\hat{V}^\top   } \rbra{\alpha(t)x_0 - \hat{V} b_t}   }^2.
%\end{equation}

%The solution is 
%\begin{equation}\label{equ:bt solution}
%    \hat{b}_t = \alpha(t)\hat{V}^\top \bar{x}_0.
%\end{equation}

%Substitute \eqref{equ:bt solution} in \eqref{equ:score mid},
%then $\hat{V}$ minimizes:
%\begin{equation}
%    \hat{V} =\argmin_{V^\top V = I_d} \sum_{x_{0,i}\in \cD}\int_{t_0}^T \dabs{\fs{\alpha(t)}{h(t)}\rbra{I - \alpha^2(t) V V^\top}\rbra{x_{0,i} - VV^\top \Bar{x}_0}}^2 \dif t.
%\end{equation}







    
% \end{proof}










\subsection{Proof of \cref{thm:w.o.subspace}}\label{pf:w.o.subspace}
\begin{proof}
The proof is a special case of Theorem~\ref{thm:w.o. update w. subspace} in Appendix~\ref{sec:proof of opt theorem}, via setting the representation matrix $A = I_D$.
\end{proof}

%Set $A = I_{D}$, \cref{thm:w.o. update w. subspace} interprets \cref{thm:w.o.subspace}. See the proof of \cref{thm:w.o. update w. subspace} in \cref{sec:proof of opt theorem}

\subsection{Proof of Theorem~\ref{thm:w.o. update w. subspace}} \label{sec:proof of opt theorem}



%For the sake of convenience, we combine the proofs of Theorems \ref{thm:w.o. update w. subspace} and \ref{thm:w. update w. subspace} and present them together. For \cref{thm:w. update w. subspace}, we set batch size as 1 for generation in each round.






%For Alg.\ref{alg:main} and Alg.\ref{alg:main_w_update}, $z_k \in \operatorname{Span}(A), \forall i \in [K]$ according to  Lemma \ref{lmm:backward process solution}.



%First, for \cref{thm:w.o. update w. subspace}, 
%\begin{equation*}
 %   \begin{aligned}
  %      w_k^0 &= 1 \\
   %     w_k^i  &= 0. \quad \forall 1\leq i \leq k.
   % \end{aligned}
%\end{equation*}
%Denote $w_{k,1} = w_{k}^k = 0$ for \cref{thm:w.o. update w. subspace}.


%As for \cref{thm:w. update w. subspace}, we set
%\begin{equation*}
 %   \begin{aligned}
  %      w_k^k &= w_{k,2},\\
   %     w_k^i &= 0, \quad \forall 1 \leq i \leq k-1; \\
    %    w_k^0 &= 1 - w_{k,2}.
   % \end{aligned}
%\end{equation*}



%Considering Lemma \ref{lmm:backward process solution}, we set $y_k, \eta, w_k$ as follows, for Theorem \ref{thm:w.o. update w. subspace},
%\begin{align}
%    y_k &= c_1^{-1}\rbra{\gamma_k,A^\top g_k} \rbra{ \fs{1}{\lambda}-c_2\rbra{\gamma_k,A^\top g_k} g_k^\top A \Bar{x}_0 }, \label{equ:y_k for w.o. update} \\
 %   \eta_1 &= \fs{1}{\lambda}, \\
 %   w_{k,1} &= 0;
%\end{align}


%for Theorem \ref{thm:w. update w. subspace},
%\begin{align}
%    y_k &= c_1^{-1}\rbra{\gamma_k,A^\top g_k} \rbra{ \fs{2}{L +2\lambda}-c_2\rbra{\gamma_k,A^\top g_k} g_k^\top A \rbra{(1-w_k)\Bar{x}_0+w_k z_k} }, \label{equ:y_k for w. update}\\
 %   \eta_2 &= \fs{2}{L+2\lambda}, \\
 %   w_{k,2} &= \fs{L}{L+2\lambda}.
%\end{align}


%For both it holds,
%\begin{equation*}
%    1 - w_{k,i} = \eta_i \lambda, \quad i \in \cbra{1,2}.
%\end{equation*}
%In the forthcoming proofs, for the sake of simplicity, we consistently use $w_k$ to denote $w_{k,i}$, and $\eta$ for $\eta_{i}$, $i \in \cbra{1,2}$. Furthermore, denote
%\begin{equation*}
 %   \zeta := \rbra{1 - (L+\lambda)\eta}^2.
%\end{equation*}


%According to \eqref{equ:sample mean} in Lemma \ref{lmm:backward process solution} and the seletion of $y_k$, the iterate $z_k$ follows 
%\begin{equation*}
%    \begin{aligned}
 %       \EE z_k = A A^\top \rbra{\Bar{x}_k + \eta  \nabla f(z_{k-1}) }
 %   \end{aligned}
%\end{equation*}


%where 
%\begin{equation*}
%    \Bar{x}_k = (1-w_k)\Bar{x}_0 + w_k z_{k-1},
%\end{equation*}

%if not updating pre-trained score, then $w_k = 0$. The mean of iterate $z_k$ can be rearranged as
%\begin{equation*}
%    \begin{aligned}
 %       \EE z_k &= AA^\top \sbra{z_{k-1} - (1-w_k)\rbra{z_{k-1}- \Bar{x}_0} + \eta \nabla f(z_{k-1})  } \\
  %      &= AA^\top \rbra{z_{k-1} + \eta \nabla h_{\lambda}(z_{k-1})  }, 
  %  \end{aligned}
%\end{equation*}
%the last line is because $1 - w_k = \eta \lambda $.





\begin{proof}[Proof of Theorem~\ref{thm:w.o. update w. subspace}]
Define a filtration $\cbra{\cH_k}_{k=0}^{K-1}$ with $\cH_k$ be the information accumulated after $k$
rounds of Alg.\ref{alg:main}.
\begin{equation*}
\begin{aligned}
      \cH_0 &:= \sigma (\bar{x}_0), \\
      \cH_k &:= \sigma \rbra{\cH_{k-1}, \sigma \rbra{z_{k-1,1}, \ldots, z_{k-1,B_{k-1}}} }, \quad k \in [K-1].
\end{aligned}
\end{equation*}
Define the expectation of samples at $k$ round as
\begin{equation*}
    \tilde{z}_{k} := \EE [z_{k,i} \mid \cH_{k-1}], \quad k \in [K-1].
\end{equation*}
If we set $y_k$ as follows 
\begin{equation*}
    y_k = \eta \cdot \rbra{\sigma^2 + g_k^\top AA^\top g_k } + g_k^\top AA^\top \bar{x}_0,
\end{equation*}
where $\eta > 0$ will be specified later. Then, according to Lemma~\ref{lmm:posterior distribution}, the sample $z_{k,i}$ follows
\begin{equation*}
   \tilde{z}_k =  \EE [z_{k,i} \mid \cH_{k-1}] = AA^\top \bar{x}_0 + \eta  \cdot A A^\top   g_{k-1},
\end{equation*}
where $g_{k-1} = \nabla f \rbra{\bar{z}_{k-1}}$ and $\bar{z}_{k-1} =  \rbra{1/B} \sum_i^B z_{k-1, i} $. We rearrange the update rule to show a gradient ascent formula as follows
\begin{equation*}
\begin{aligned}
   \tilde{z}_k &= AA^\top \tilde{z}_{k-1} - AA^\top \rbra{\tilde{z}_{k-1} - \bar{x}_0 } +  \eta  \cdot A  A^\top   \nabla f(\tilde{z}_{k-1}) + \eta  \cdot A A^\top  \rbra{ g_{k-1}-\nabla f(\tilde{z}_{k-1})}\\
    &= AA^\top \tilde{z}_{k-1} - A A^\top A A^\top \rbra{\tilde{z}_{k-1} - \bar{x}_0 } +  \eta  \cdot A  A^\top   \nabla f(\tilde{z}_{k-1}) + \eta  \cdot A  A^\top  \rbra{ g_{k-1}-\nabla f(\tilde{z}_{k-1})} \\
    &= AA^\top \tilde{z}_{k-1} + \eta  \cdot A A^\top   \nabla h(\tilde{z}_{k-1}) + \eta  \cdot A A^\top  \rbra{ g_{k-1}-\nabla f(\tilde{z}_{k-1})},
\end{aligned}
\end{equation*}
where $h(x) := f(x) - \lambda / 2 \dabs{x - \bar{x}_0}^2 $, $\lambda = 1/ \eta$. Recall the notation for the optimum: $x^\star_{A,\lambda} = \argmax_{x=Au} h(x)$. All samples and expectations lying in the subspace according to Lemma~\ref{lmm:sample in subspace}, we consider the distance of the latent variables in the subspace under norm $\dabs{\cdot}_2$.
\begin{align}
    \dabs{AA^\top \rbra{\tilde{z}_k  - x^\star_{A,\lambda} } }^2 &= \dabs{AA^\top \rbra{\tilde{z}_{k-1} - x^\star_{A,\lambda}} + \eta A A^\top   \nabla h(\tilde{z}_{k-1}) + \eta A A^\top  \rbra{ g_{k-1}-\nabla f(\tilde{z}_{k-1})}}^2 \nonumber \\
    & \leq 2 \cdot \underbrace{\dabs{AA^\top \rbra{\tilde{z}_{k-1} - x^\star_{A,\lambda}} + \eta AA^\top   \nabla h(\tilde{z}_{k-1})}^2}_{:= I_1} + 2 \cdot \underbrace{\dabs{ \eta A A^\top  \rbra{ g_{k-1}-\nabla f(\tilde{z}_{k-1})}}^2}_{:= I_2}. \label{equ:distance two terms to bound}
\end{align}
We bound the second term $I_2$ firstly. 
\begin{equation*}
    \begin{aligned}
         I_2 = \eta^2   \dabs{ AA^\top  \rbra{ g_{k-1}-\nabla f(\tilde{z}_{k-1})}}^2 
         \leq \eta^2   \dabs{ g_{k-1}-\nabla f(\tilde{z}_{k-1})}^2  \leq \eta^2  L^2  \dabs{ \bar{z}_{k-1}-\tilde{z}_{k-1}}^2,
    \end{aligned}
\end{equation*}
where the last inequality is derived from  $L$-smoothness of $f$. Lemma~\ref{lmm:posterior distribution} shows the distribution of $z_{k-1,i}$. Therefore, according to concentration inequality for Gaussian distribution $A^\top z_{k-1,i}$, with the probability at least $1 - \delta / K $, it holds $$\dabs{A^\top \bar{z}_{k-1} - A^\top \tilde{z}_{k-1}}^2 \leq 2 \log \rbra{\frac{2dK}{\delta}} \cdot \fs{\text{trace}\rbra{\VV(z_{k-1,i})}}{B_{k-1}} \leq 2 \log \rbra{\frac{2dK}{\delta}} \cdot \fs{d}{B_{k-1}}  .$$ 
Consider ${z}_{k-1,i} \in \operatorname{Span}(A)$ due to Lemma~\ref{lmm:sample in subspace}, we have $ \dabs{\bar{z}_{k-1} -  \tilde{z}_{k-1}}^2 = \dabs{A^\top \bar{z}_{k-1} - A^\top \tilde{z}_{k-1}}^2 $. Therefore, $I_2$ is bounded by $$I_2 \leq d M_0 /B_{k-1}, $$ where $M_0:= 2\eta^2  L^2 \log \rbra{\frac{2dK}{\delta}} $.
Next, we consider the first term in \eqref{equ:distance two terms to bound}. Since $x^*_{A,\lambda}$ is the optimum of $h$ within $\operatorname{Span}(A)$, the gradient $\nabla h(x^*_{A,\lambda})$ is in the orthogonal subspace, i.e., $A^\top \nabla h(x^*_{A,\lambda}) = 0 $. The first term in \eqref{equ:distance two terms to bound} can be written as
\begin{equation*}
    \begin{aligned}
         I_1 &= \dabs{AA^\top\sbra{\tilde{z}_{k-1} - x^\star_{A,\lambda} + \eta \rbra{\nabla h(\tilde{z}_{k-1})-\nabla h(x^*_{A,\lambda})}}}^2 \\
         & \leq  \dabs{\tilde{z}_{k-1} - x^\star_{A,\lambda} + \eta \rbra{\nabla h(\tilde{z}_{k-1})-\nabla h(x^*_{A,\lambda})}}^2 \\
        &=  \dabs{\tilde{z}_{k-1}  - x^\star_{A,\lambda} }^2+ \dabs{\eta  \rbra{\nabla h(\tilde{z}_{k-1})-\nabla h(x^*_{A,\lambda})}}^2 \\
        & \quad + 2 \pbra{\tilde{z}_{k-1} - x^\star_{A,\lambda},   \eta  \rbra{\nabla h(\tilde{z}_{k-1})-\nabla h(x^*_{A,\lambda})} }. 
    \end{aligned}
\end{equation*}
Recall $h$ is $f$ adding a regularized term. We get $h$ is $(L+ \lambda)$-smooth and $\lambda $-strongly concave.  According to Lemma~\ref{lmm:opt}, we derive
\begin{equation*}
    \begin{aligned}
        \pbra{\tilde{z}_{k-1} - x^\star_{A,\lambda},   \nabla h(\tilde{z}_{k-1})-\nabla h(x^*_{A,\lambda})} \leq - \fs{\lambda(L+ \lambda)}{L+ 2\lambda } \dabs{\tilde{z}_{k-1} - x^*_{A,\lambda}}^2  - \fs{1}{L+ 2\lambda } \dabs{\nabla h(\tilde{z}_{k-1})-\nabla h(x^*_{A,\lambda})}^2.
    \end{aligned}
\end{equation*}
Plugin the formula of $I_1$, we get
\begin{equation*}
    \begin{aligned}
        I_1 \leq \rbra{1 - \fs{2\eta \lambda(L+ \lambda)}{L+ 2\lambda } } \dabs{\tilde{z}_{k-1}  - x^\star_{A,\lambda}  }^2+ \rbra{\eta^2 - \fs{2\eta}{L + 2\lambda}}\dabs{\nabla h(\tilde{z}_{k-1})-\nabla h(x^*_{A,\lambda})}^2 .
    \end{aligned}
\end{equation*}
Recall $\eta = 1/\lambda$, thus we have $\eta^2 - \fs{2\eta}{L + 2\lambda} > 0$. Since $h$ is $(L+\lambda)$-smooth, we have $\dabs{\nabla h(\tilde{z}_{k-1})-\nabla h(x^*_{A,\lambda})} \leq (L+\lambda)\dabs{\tilde{z}_{k-1}- x^*_{A,\lambda}}$. Therefore, we get
\begin{equation*}
    I_1 \leq \zeta \dabs{\tilde{z}_{k-1}  - x^\star_{A,\lambda}  }^2
\end{equation*}
where $\zeta:= \rbra{1-\eta(L+\lambda)}^2 $.
Combing the upper bound of $I_1$ and $I_2$, we get with probability at least $1 - \delta/K$, for $1 < k \leq K$,
\begin{equation*}
     \dabs{\tilde{z}_{k}  - x^\star_{A,\lambda} }^2 \leq \zeta  \dabs{\tilde{z}_{k-1}  - x^\star_{A,\lambda}  }^2 + \fs{d M_0}{B_{k-1}}.
\end{equation*}
where we use $x^*_{A,\lambda}, \tilde{z}_{k-1} \in \operatorname{Span}(A)$ due to Lemma~\ref{lmm:sample in subspace}, thus $AA^\top (\tilde{z}_{k} - x^*_{A,\lambda}) = \tilde{z}_{k} - x^*_{A,\lambda} $.
As for $k=1$, by similar derivation, we can obtain $\dabs{\tilde{z}_{1}  - x^\star_{A,\lambda} }^2 \leq \zeta  \dabs{\bar{z}_{0}  - x^\star_{A,\lambda} }^2$.
By induction, we get with probability at least $1 - \rbra{(K-1)/K}\delta$, 
\begin{equation*}
    \begin{aligned}
    \dabs{\tilde{z}_{K}  - x^\star_{A,\lambda} }^2 \leq \zeta^K  \dabs{\bar{z}_{0}  - x^\star_{A,\lambda}  }^2  + d M_0 \sum_{k=1}^{k-1}\fs{\zeta^{K-k-1}}{B_k}.
    \end{aligned}
\end{equation*}
Since $\dabs{\bar{z}_{K} -  \tilde{z}_{K}}^2 \leq d M_0 /B_K$, we have with probability at least $1 - \delta$, 
\begin{equation*}
\begin{aligned}
    \dabs{\bar{z}_{K} -  x^\star_{A,\lambda}} &\leq \dabs{\tilde{z}_{K}  - x^\star_{A,\lambda}  } + \dabs{ \bar{z}_{K} -  \tilde{z}_{K}} \\
    &\leq \sqrt{\zeta^K  \dabs{\bar{z}_{0}  - x^\star_{A,\lambda}  }^2  + d M_0 \sum_{k=1}^{k-1}\fs{\zeta^{K-k-1}}{B_k}} + \sqrt{\fs{d M_0}{B_K}} \\
    &\leq \zeta^{K/2}  \dabs{\bar{z}_{0}  - x^\star_{A,\lambda}  } + 2 \sqrt{d M_0 \sum_{k=1}^{k-1}\fs{\zeta^{K-k-1}}{B_k} + \fs{d M_0}{B_K }}
\end{aligned}
\end{equation*}
Choose $B_k \geq \zeta^{-2k-1} $ for all $k \in [K]$, then we can get 
\begin{equation}\label{equ:final iter distance}
    \dabs{\bar{z}_{K} -  x^\star_{A,\lambda}} \leq \zeta^{K/2} \rbra{\dabs{\bar{z}_{0}  - x^\star_{A,\lambda}  } + 2 \sqrt{d M_1 } }
\end{equation}
where $M_1 := (1-\zeta)^{-1} M_0 $.
Since $h$ is $(L + \lambda)$-smooth, it holds
\begin{equation*}
    \abs{h(\bar{z}_{K}) - h(x^*_{A,\lambda}) - \pbra{\nabla h(x^*_{A,\lambda}), \bar z_{K} - x^*_{A,\lambda}}} \leq \fs{L + \lambda}{2} \dabs{\bar z_{K} - x^*_{A,\lambda}}^2. 
\end{equation*}
Considering that $\nabla h(x^*_{A,\lambda}) \perp \operatorname{Span}(A) $ yields $\pbra{\nabla h(x^*_{A,\lambda}), \bar z_{K} - x^*_{A,\lambda}} = 0$, we obtain the following by rearranging the equation above
\begin{align}
       f\rbra{x^*_{A,\lambda}} - f(\bar z_K)  &\leq  \fs{\lambda}{2}\rbra{\dabs{x^*_{A,\lambda}-\Bar{x}_0}^2 -\dabs{\bar z_K - \Bar{x}_0}^2}  + \fs{L + \lambda }{2} \dabs{\bar z_{K} - x^*_{A,\lambda}}^2  \label{equ:rearrange smooth} \\
       &\leq \sbra{\lambda \dabs{\Bar{x}_0 - x^*_{A,\lambda}}\dabs{z_{K} - x^*_{A,\lambda}} + (L+\lambda)\dabs{z_{K} - x^*_{A,\lambda}}^2 } . \nonumber
\end{align}
Substitute \eqref{equ:final iter distance} into above upper bound, and we have with probability at least $1 - \delta$, 
\begin{equation*}
    \begin{aligned}
        f\rbra{x^*_{A,\lambda}} - f(\bar z_K)  \lesssim  \zeta^{K/2} \cdot (L + \lambda ) \sbra{\dabs{\Bar{x}_0 - x^*_{A,\lambda}}^2 + \dabs{\Bar{z}_0 - x^*_{A,\lambda}}^2 + dM_1 }. 
    \end{aligned}
\end{equation*}
According to the Assumption \ref{asmp:subspace_data}, the mean of data is also in the subspace $A$, together with $x^*_{A,\lambda} \in \operatorname{Span}(A)$ and $\bar{z}_0 = \bar{x}_0$, we have $\dabs{\Bar{x}_0 - x^*_{A,\lambda}}^2 + \dabs{\Bar{z}_0 - x^*_{A,\lambda}}^2 = \cO(d)$. Therefore, we get the final result.
\end{proof}











==> neurips/appdicies/proof_lemmas.tex <==
\section{Additional Lemmas}\label{app:additional lmm}
In this section, we provide supplementary lemmas to complement the main content. The subsequent lemma shows unconditional score adding guidance $\texttt{G}_{loss} $ to retrieve the conditional score under the Gaussian data and linear rewards setting. 

\begin{lemma}\label{lmm:recover condi score}
Suppose $X_0 \sim \cN \rbra{\mu, \Sigma }, Y = g^\top X_0 + \epsilon $ where $\epsilon \sim \cN (0, \sigma^2)$ is independent with $X_0$. $\cbra{X_t}_{t \ge 0} $ is the stochastic process from the forward process. Then, 
\begin{equation*}
    \nabla \log p_t(x_t) + \texttt{G}_{loss}(x_t,t) = \nabla_{x_t} \log p_t(x_t \mid y),
\end{equation*}
with $\beta(t)$ specified as
\begin{equation*}
    \beta(t) = \fs{1}{2} \sbra{\sigma^2 + g^\top \Sigma^{-1}  \rbra{ I_D + \fs{\alpha^2(t)}{h(t)} \Sigma }^{-1} g     }^{-1},
\end{equation*}
where $\Sigma^{-1}$ is the Moore–Penrose inverse of $\Sigma$.
\end{lemma}
\begin{proof}
  Since $X_0, X_t$ and $Y$ are joint Gaussian, we have $Y \mid X_t$ also follows Gaussian distribution, denoted as $\cN \rbra{m_y(x_t), \sigma_y^2(x_t)}$.Then, the closed form of $\nabla_{x_t} \log p_t(y \mid x_t)  $ can be derived  as
\begin{equation*}
    \nabla_{x_t} \log p_t(y \mid x_t) = - \nabla_{x_t} \sbra{\fs{1}{2}\rbra{\frac{y - m_y(x_t) }{\sigma_y(x_t)}}^2 } - \nabla_{x_t} \log \sigma_y(x_t).
\end{equation*}
Due to the linearity of $Y$ with regard to $X_0$, $m_y(x_t)$ can be computed as
\begin{equation}\label{equ:mean of y on xt}
    \begin{aligned}
        m_y(x_t) = \EE [y \mid x_t] = \EE [g^\top x_0 + \epsilon \mid x_t] = \EE [g^\top x_0  \mid x_t] = g^\top \EE [ x_0  \mid x_t]. 
    \end{aligned}
\end{equation}
To get the variance $\sigma_y^2(x_t)$, we compute the joint distribution $(X_t, Y)$. In the forward process, given $X_0 = x_0$, $X_t$ can be written as $\alpha(t) x_0 + Z_t$ for $Z_t \sim \cN(0, h(t)I_D)$ independent of $x_0$. Due to the linear function assumption, we have
\begin{align*}
\begin{bmatrix}
X_t \\
Y
\end{bmatrix}
=
\begin{bmatrix}
\alpha(t)I_D & 0 & I_D \\
g^\top & 1 & 0
\end{bmatrix}
\begin{bmatrix}
x_0 \\
\epsilon \\
Z_t
\end{bmatrix}.
\end{align*}
Observing that the joint distribution of $(x_0, \epsilon, z_t)$ is Gaussian, we deduce
\begin{align*}
\begin{bmatrix}
X_t \\
Y
\end{bmatrix}
\sim \cN\left(
\begin{bmatrix}
\alpha(t) \mu \\
g^\top \mu
\end{bmatrix},
\begin{bmatrix}
\alpha^2(t) \Sigma + h(t) I_D & \alpha(t) \Sigma g \\
\alpha(t)g^\top \Sigma & \sigma^2 + g^\top \Sigma g
\end{bmatrix}\right).
\end{align*}
Thus, we get $\sigma_y^2(x_t) = \sigma^2 + g^\top \Sigma g - \alpha^2(t) g^\top \Sigma \rbra{\alpha^2(t) \Sigma + h(t) I_D }^{-1} \Sigma g  $. Together with the derivation of the mean $m_y(x_t)$ \eqref{equ:mean of y on xt}, we get
\begin{equation*}
    \nabla_{x_t} \log p_t(y \mid x_t) = - \fs{1}{2 \sigma_y^2(x_t)  } \nabla_{x_t} \sbra{\rbra{y - g^\top \EE [ x_0  \mid x_t]}^2 }.
\end{equation*}
Recall the definition of $\texttt{G}_{loss}$ \eqref{equ:gradient_guidance+}, and we get $\texttt{G}_{loss}(x_t,t) = \nabla_{x_t} \log p_t(y \mid x_t)$ if $\beta(t)$ is specified as
\begin{equation*}
\begin{aligned}
    \beta(t) &= \rbra{2 \sigma_y^2(x_t)}^{-1} = \rbra{2\rbra{\sigma^2 + g^\top \Sigma g - \alpha^2(t) g^\top \Sigma \rbra{\alpha^2(t) \Sigma + h(t) I_D }^{-1} \Sigma g}}^{-1} \\
    &= \fs{1}{2} \sbra{\sigma^2 + g^\top \Sigma^{-1}  \rbra{ I_D + \fs{\alpha^2(t)}{h(t)} \Sigma }^{-1} g }^{-1}.
\end{aligned}
\end{equation*}
The proof is completed.
\end{proof}









%\yingqing{give a proof?}


























==> neurips/appdicies/proof_score_match.tex <==
\subsection{Proof of Lemma~\ref{lmm:fully score matching}}\label{prof:fully score matching}

\begin{lemma}
\label{lmm:fully score matching}
Suppose for pre-training the score network, the class in \eqref{equ:score match objective} is
\begin{equation}
\cS = \cbra{s(x, t)= - C_t x + b_t : C_t \in \RR^{D\times D}, \, b_t \in \RR^D}.
\end{equation}
Let $\cD$ be the pre-training data. Minimizing the score matching objective \eqref{equ:score match objective} over the function class \eqref{equ:fully linear class} gives 
\begin{equation}%\label{equ:pre-train score solution fully linear}
{s}_{\theta}(x_t,t)= - \rbra{\alpha^2(t) \Bar{\Sigma} + h(t)I_D }^{-1}\rbra{ x_t - \alpha(t)\bar{\mu}},
\end{equation}
where $\bar{\mu} = {\EE}_{x\in \cD}[x]$ and $\Bar{\Sigma} = {\EE}_{x\in \cD} \sbra{(x-\bar{\mu}) (x-\bar{\mu})^\top} $ are data mean and covariance, respectively. 
\end{lemma}



\begin{proof}
Using the linear score network class $\cS$, we cast the score matching loss \eqref{equ:score match objective} into
\begin{align*}
& \quad \int_{0}^{T} \hat{\EE}_{x_0 \in \mathcal{D}} \EE_{x_t\sim\cN\rbra{\alpha(t)x_0,h(t)I_D}}  \sbra{\dabs{\nabla_{x_t} \log \phi_t(x_t|x_0)-s(x_t, t)}^2} \dif t \\
& = \int_{0}^{T} \hat{\EE}_{x_0 \in \mathcal{D}} \EE_{x_t\sim\cN\rbra{\alpha(t)x_0,h(t)I_D}}  \sbra{\dabs{-\frac{1}{h(t)} (x_t - \alpha(t)x_0) + C_tx_t - b_t}^2} \dif t \\
& = \int_{0}^{T} \hat{\EE}_{x_0 \in \mathcal{D}} \EE_{x_t\sim\cN\rbra{\alpha(t)x_0,h(t)I_D}}  \sbra{\dabs{\left(C_t-\frac{1}{h(t)}I_D \right)(x_t - \alpha(t)x_0) + (\alpha(t)C_tx_0 - b_t)}^2} \dif t \\
& \overset{(i)}{=} \int_{0}^{T} \hat{\EE}_{x_0 \in \mathcal{D}} \left[\dabs{b_t - \alpha(t)C_tx_0}^2\right] + \int_{0}^{T} \text{trace}\rbra{ h(t) \left(C_t - \frac{1}{h(t)}I_D\right)^\top\left(C_t - \frac{1}{h(t)}I_D\right) }\dif t,
\end{align*}
where equality $(i)$ follows from computing the expectation over the conditional Gaussian distribution of $x_t | x_0$. We note that $b_t$ should minimize $\hat{\EE}_{x_0 \in \mathcal{D}} \left[\dabs{b_t - \alpha(t)C_tx_0}^2\right]$ for any $t$, which leads to
\begin{align*}
\hat{b}_t = \alpha(t) C_t \bar{x}_0.
\end{align*}
Substituting $\hat{b}_t$ into the optimization objective \eqref{equ:score match objective} yields:
\begin{equation*}
    \begin{aligned}
        & \quad  \int_{0}^{T} \hat{\EE}_{x_0 \in \mathcal{D}} \left[\dabs{\alpha(t) C_t \bar{x}_0 - \alpha(t)C_tx_0}^2\right] + \int_{0}^{T} \text{trace}\rbra{  h(t) \left(C_t - \frac{1}{h(t)}I_D\right)^\top\left(C_t - \frac{1}{h(t)}I_D\right)}\dif t \\
        &= \int_{0}^{T} \alpha^2(t)\hat{\EE}_{x_0 \in \mathcal{D}}  \left[\dabs{ C_t (x_0 - \bar{x}_0)}^2\right] + \int_{0}^{T} \text{trace}\rbra{ h(t) \left(C_t^\top C_t - \fs{1}{h(t)}C_t -  \fs{1}{h(t)}C_t^\top + \fs{1}{h^2(t)}I_D\right)}\dif t. \\
    \end{aligned}
\end{equation*}
Taking the gradient for $C_t$, we get
\begin{equation*}
    2 \alpha^2(t) C_t \hat{\EE}_{x_0 \in \mathcal{D}} \sbra{(x_0 - \bar{x}_0) (x_0 - \bar{x}_0)^\top} + 2h(t) C_t - 2I_D.
\end{equation*}
Thus, we get the solution for $\hat C_t$ as
\begin{equation*}
    \hat{C}_t = \rbra{\alpha^2(t) \hat{\EE}_{x_0 \in \mathcal{D}} \sbra{(x_0 - \bar{x}_0) (x_0 - \bar{x}_0)^\top} + h(t)I_D}^{-1}.
\end{equation*}
Therefore, optimizing \eqref{equ:score match objective} over linear score network class $\cS$ gives rise to
\begin{equation*}
{s}_{\theta}(x_t,t)= - \rbra{\alpha^2(t) \Bar{\Sigma}_{0} + h(t)I_D }^{-1}\rbra{ x_t - \alpha(t)\bar{x}_0}.
\end{equation*}

\end{proof}


==> neurips/appdicies/proof_sec6.tex <==
\section{Omitted Proof of Theorem~\ref{thm:w. update w. subspace}} \label{sec:proof of opt theorem update}
\begin{proof}
Define
\begin{equation*}
    \begin{aligned}
      \cH_0 &:= \sigma (\bar{x}_0), \\
      \cH_k &:= \sigma \rbra{\cH_{k-1}, \sigma \rbra{z_{k-1,1}, \ldots, z_{k-1,B_{k-1}}} }, \quad k \in [K-1], \\
      \tilde{z}_{k} &:= \EE [z_{k,i} \mid \cH_{k-1}], \quad k \in [K-1].
\end{aligned}
\end{equation*}
We notice Lemma~\ref{lmm:general weights score match} gives the formula of the pre-trained score in each iteration, thus applying Lemma~\ref{lmm:posterior distribution} with replacing $\bar{x}_0$ with $\bar{z}_{k-1}^w := \sum_{j=0}^{k-1} w_{k-1}^j \bar{z}_j $ yields the distribution of $z_{k,i}$. We get
\begin{equation*}
    \tilde{z}_k = AA^\top \bar{z}_{k-1}^w +   \frac{y_{k-1} - g_{k-1}^\top AA^\top \bar{z}_{k-1}^w}{\sigma^2 + g_{k-1}^\top AA^\top g_{k-1}} AA^\top g_{k-1}.
\end{equation*}
We choose $y_{k-1}$ and weights $w_{k-1}^j$ as
\begin{equation*}
    \begin{aligned}
        y_{k-1} &= \eta_{k-1} \cdot \rbra{\sigma^2 + g_{k-1}^\top AA^\top g_{k-1}} + g_{k-1}^\top AA^\top \bar{z}_{k-1}^w,\\
        w_{k-1}^0 &= 1 - w_{k-1} \\
        w_{k-1}^j &= 0 , \,\, 1 \leq j < k-1, \\
        w_{k-1}^{k-1} &= w_{k-1},
    \end{aligned}
\end{equation*}
where $\eta_{k-1} > 0$, $0<w_{k-1}<1$ will be specified later. Thus, the update rule reduce to
\begin{equation*}
    \begin{aligned}
        \tilde{z}_k &= AA^\top \rbra{(1-w_{k-1})\bar{x}_0 + w_{k-1}\bar{z}_{k-1} + \eta_{k-1} g_{k-1}} \\
        &=  AA^\top \sbra{\bar{z}_{k-1} + \eta_{k-1} \rbra{\nabla f(\bar{z}_{k-1}) - \eta_{k-1}^{-1}(1-w_{k-1})\rbra{\bar{z}_{k-1} - \bar{x}_0} }}.
    \end{aligned}
\end{equation*}
We set $w_{k-1} = 1- \eta_{k-1} \lambda$ and set $\eta_{k-1} = \eta =  2/(L+2\lambda)$, where $\lambda > 0$. Therefore, we have
\begin{equation}\label{equ:shrink distance}
    \begin{aligned}
        \tilde{z}_k =  AA^\top \rbra{\bar{z}_{k-1} + \eta \nabla h_{\lambda}(\bar{z}_{k-1})},
    \end{aligned}
\end{equation}
where $h_{\lambda}(x):= f(x) - (\lambda/2) \dabs{x - \bar{x}_0 }^2 $. Define $ x^\star_{A,\lambda} = \argmax_{x=Au} h_{\lambda}(x) $. With some similar steps in proof in Appendix~\ref{sec:proof of opt theorem}, we get
\begin{equation*}
    \dabs{\bar{z}_{K} -  x^\star_{A,\lambda}} \leq \zeta^{K/2} \rbra{\dabs{\bar{z}_{0}  - x^\star_{A,\lambda}  } + 2 \sqrt{d M_1 } }, \quad \text{w.p.} \,\,  1- \delta,
\end{equation*}
where $\zeta = \rbra{1-\eta(L+\lambda)}^2 = L^2 / (L+2\lambda)^2 $ and $M_1 = (1-\zeta)^{-1} \cdot 4(1+\eta^2)L^2 \log \rbra{\fs{2dK}{\delta}}$. Also, we can get \eqref{equ:rearrange smooth} as in proof in Appendix~\ref{sec:proof of opt theorem}. We restate it here:
\begin{equation}\label{equ:restate rearrange smooth}
    f\rbra{x^*_{A,\lambda}} - f(\bar z_K)  \leq  \fs{\lambda}{2}\rbra{\dabs{x^*_{A,\lambda}-\Bar{x}_0}^2 -\dabs{\bar z_K - \Bar{x}_0}^2}  + \fs{L + \lambda }{2} \dabs{\bar z_{K} - x^*_{A,\lambda}}^2.
\end{equation}
Since $f$ is concave,
\begin{equation*}
    \begin{aligned}
       f\rbra{x_{A}^\ast} -  f\rbra{x^*_{A,\lambda}} \leq \pbra{\nabla  f\rbra{x^*_{A,\lambda}}, x_{A}^\ast-x^*_{A,\lambda}} = \lambda \pbra{x^*_{A,\lambda}-\Bar{x}_0, x_{A}^\ast-x^*_{A,\lambda}}.
    \end{aligned}
\end{equation*}
Adding \eqref{equ:restate rearrange smooth}, it holds
\begin{equation*}
    \begin{aligned}
        f\rbra{x^*_{A,\lambda}} - f(\bar z_K) &\leq  \sbra{\fs{\lambda}{2}\rbra{\dabs{x_{A}^\ast - \Bar{x}_0}^2 - \dabs{x^*_{A,\lambda}-x_{A}^\ast}^2-\dabs{\bar z_K - \Bar{x}_0}^2}  + \fs{\lambda+L}{2} \dabs{\bar z_{K} - x^*_{A,\lambda}}^2 }.
    \end{aligned}
\end{equation*}
Due to \eqref{equ:shrink distance} and $\bar{z}_0 = \bar{x}_0$, we have
\begin{equation*}
    f\rbra{x^*_{A,\lambda}} - f(\bar z_K) \lesssim  \sbra{\lambda {\dabs{x_{A}^\ast - \Bar{x}_0}^2 } + (L+\lambda) \zeta^K \rbra{\dabs{\Bar{x}_{0} - x^*_{A,\lambda}}^2 + d M_1 } }, \,\,  1- \delta.
\end{equation*}
We choose $\lambda = L \log K /(4K)$ and get
\begin{equation*}
\begin{aligned}
    f\rbra{x^*_{A,\lambda}} - f(\bar z_K) &\lesssim \fs{L\log K}{K} \cdot \sbra{\dabs{x_{A}^\ast - \Bar{x}_0}^2 +\dabs{\Bar{x}_{0} - x^*_{A,\lambda}}^2 + d M_1 }, \,\,  1- \delta.
\end{aligned}
\end{equation*}
With assuming $\dabs{x^\star_{A}}$ is bounded thus $\dabs{x^\star_{A,\lambda}}$ is bounded, we derive
\begin{equation*}
    f\rbra{x^*_{A,\lambda}} - f(\bar z_K) = O \rbra{\fs{L\log K}{K} d}, \,\,  1- \delta.
\end{equation*}











\end{proof}

==> neurips/appdicies/proofs_new.tex <==
\section{Omitted Proofs in \cref{sec:grad_guidance}}
\yingqing{to reorganize appendix}

\DoToC
Throughout the proof, we omit the subscript $x_t$ of $\nabla$ in score function $\nabla \log p_t(x_t)$ and conditional score function $\nabla \log p_t(x_t | y)$.
\subsection{Proof of Lemma~\ref{lmm:guidance=cond w.o.subspace}}
\label{prf:lmm:guidance=cond w.o.subspace}
\begin{proof}%\yingqing{adding proof for $\Sigma$ case, or just cite lemma 13}
Under the assumption of initial data distribution $X \sim \cN(\mu, I_D)$, we can check that the marginal distribution of $X_t$ for any $t \in [0, T]$ is also Gaussian. Indeed, utilizing the transition in the forward process \eqref{eq:forward_sde}, we derive
\begin{align*}
p_t(x_t) & = \int_{x_0} \phi_t(x_t | x_0) p_0(x_0) \diff x_0 \\
& = \int_{x_0} \frac{1}{(2\pi h(t))^{D/2}} \exp\left(-\frac{1}{2h(t)} \dabs{x_t - \alpha(t)x_0}^2\right) \frac{1}{(2\pi)^{D/2}} \exp\left(-\frac{1}{2} \dabs{x_0 - \mu}^2\right) \diff x_0 \\
& = \frac{1}{(2\pi)^{D/2}} \exp\left(-\frac{1}{2} \dabs{x_t - \alpha(t)\mu}^2\right).
\end{align*}
Therefore, the unconditioned score function $\nabla \log p_t(x_t)$ is
\begin{align*}
\nabla \log p_t(x_t) = -(x_t - \alpha(t) \mu).
\end{align*}
The next step is to find the conditional score function $\nabla \log p_t(x_t | y)$. Remember that we only diffuse on $X_t$ but keep $y$ unchanged. Since given $X_0 = x_0$, $X_t$ can be written as $\alpha(t) x_0 + Z_t$ for $Z_t \sim \cN(0, h(t)I_D)$ independent of $x_0$. Due to the linear function assumption, we have
\begin{align*}
\begin{bmatrix}
X_t \\
Y
\end{bmatrix}
=
\begin{bmatrix}
\alpha(t)I_D & 0 & I_D \\
g^\top & 1 & 0
\end{bmatrix}
\begin{bmatrix}
x_0 \\
\epsilon \\
Z_t
\end{bmatrix}.
\end{align*}
Observing that the joint distribution of $(x_0, \epsilon, z_t)$ is Gaussian, we deduce
\begin{align*}
\begin{bmatrix}
X_t \\
Y
\end{bmatrix}
\sim \cN\left(
\begin{bmatrix}
\alpha(t) \mu \\
g^\top \mu
\end{bmatrix},
\begin{bmatrix}
I_D & \alpha(t)g \\
\alpha(t)g^\top & \dabs{g}^2+\sigma^2
\end{bmatrix}\right).
\end{align*}
The conditional distribution $X_t | Y$ can now be obtained as
\begin{align*}
X_t | Y \sim \cN\left(\alpha(t)\mu + \alpha(t) \frac{y - g^\top \mu}{\dabs{g}^2 + \sigma^2} g, I_D - \alpha^2(t) \frac{gg^\top}{\dabs{g}^2 + \sigma^2}\right).
\end{align*}
Now it is straightforward to derive the conditional score function as
\begin{align*}
\nabla \log p_t(x_t | y) & = -\left(I_D - \alpha^2(t) \frac{gg^\top}{\dabs{g}^2 + \sigma^2}\right)^{-1}\left(x_t - \alpha(t)\mu - \alpha(t) \frac{y - g^\top \mu}{\dabs{g}^2 + \sigma^2} g\right) \\
& \overset{(i)}{=} - \left(I_D + \alpha^2(t) \frac{gg^\top}{\dabs{g}^2 h(t) + \sigma^2}\right) \left(x_t - \alpha(t)\mu - \alpha(t) \frac{y - g^\top \mu}{\dabs{g}^2 + \sigma^2} g\right) \\
& = - (x_t - \alpha(t) \mu) + \alpha(t)\frac{y -g^\top \rbra{\alpha(t) x_t + h(t) \mu}  }{\sigma^2 + h(t) \dabs{g}^2} g, 
\end{align*}
where equality $(i)$ invokes the matrix inverse lemma (Woodbury matrix identity). We subtract $\nabla \log p_t(x_t)$ from $\nabla \log p_t(x_t | y)$, which leads to
\begin{align*}
\nabla \log p_t(y | x_t) & = \nabla \log p_t(x_t | y) - \nabla \log p_t(x_t) \\
& = \alpha(t)\frac{y -g^\top \rbra{\alpha(t) x_t + h(t) \mu}  }{\sigma^2 + h(t) \dabs{g}^2} g \\
& = \beta(t) \left[y - g^\top \EE[x_0 | x_t] \right]g.
\end{align*}
To see why the last equality holds, we need to verify $\EE[x_0 | x_t] = \alpha(t)x_t + h(t)\mu$. Indeed, the joint distribution of $(X_0, X_t)$ follows
\begin{align*}
\begin{bmatrix}
X_0 \\
X_t
\end{bmatrix}
\sim \cN\left(
\begin{bmatrix}
\mu \\
\alpha(t)\mu
\end{bmatrix},
\begin{bmatrix}
I_D & \alpha(t)I_D \\
\alpha(t)I_D & I_D
\end{bmatrix}
\right).
\end{align*}
Hence, the conditional expectation verifies $\EE[x_0 | x_t] = h(t)\mu + \alpha(t)x_t$. 
As for the case $X \sim \cN \rbra{\mu, \Sigma}$,  the joint distribution of $(X_0, X_t)$ follows
\begin{align*}
\begin{bmatrix}
X_0 \\
X_t
\end{bmatrix}
\sim \cN\left(
\begin{bmatrix}
\mu \\
\alpha(t)\mu
\end{bmatrix},
\begin{bmatrix}
\Sigma & \alpha(t)\Sigma \\
\alpha(t)\Sigma & \alpha^2(t)\Sigma + h(t) I_D
\end{bmatrix}
\right).
\end{align*}
We get $\EE[x_0 | x_t] =  \mu + \alpha(t) \Sigma \rbra{\alpha^2(t)\Sigma + h(t) I_D }^{-1}  \rbra{x_t - \alpha(t)\mu} $, thus $ \nabla_{x_t} \EE[x_0 | x_t] = \Sigma \rbra{\alpha^2(t)\Sigma + h(t) I_D }^{-1}$. According to the same proof of Lemma~\ref{lmm:recover condi score}, it holds $ \nabla_{x_t} \log p_t(y \mid x_t) = - \beta_1(t) \nabla_{x_t} \sbra{\rbra{y - g^\top \EE [ x_0  \mid x_t]}^2 }$ with some scalar $\beta_1(t)$. Since $\nabla_{x_t} \sbra{\rbra{y - g^\top \EE [ x_0  \mid x_t]}^2  } = - \rbra{y - g^\top \EE [ x_0  \mid x_t ]} \cdot \nabla_{x_t} \EE[x_0 | x_t] \cdot g = - \rbra{y - g^\top \EE [ x_0  \mid x_t } \cdot \rbra{\alpha^2(t)\Sigma + h(t) I_D }^{-1} \Sigma  g $.
The proof is complete.
\end{proof}

%\subsection{Proof of Lemma \ref{lmm:hat_x0}}\label{pf:hat_x0}
%\begin{proof}
%Substituting Tweedie's formula \eqref{equ:hatx0_derivation} into the definition of $\hat{\EE}[x_0 | x_t]$ in \eqref{equ:hatx0_guidance}, we obtain
%\begin{align*}
%\hat{\EE}[x_0 | x_t] = \frac{1}{\alpha(t)}(x_t + h(t) \nabla \log p_t(x_t)) = \EE[x_0 | x_t].
%\end{align*}
%The proof is complete.
%\end{proof}

\subsection{Proof of Theorem \ref{thm:faith_grad_guidance}}\label{prof:faith_grad_guidance}

%Under \ref{asmp:subspace_data}, the unconditional score is
%\begin{equation}
 %   \nabla_{x_t}p_t(x_t) = -\fs{1}{h(t)}\rbra{I - \alpha^2(t) AA^\top} x_t + \alpha(t) A \mu.
%\end{equation} 

%The conditional
%\begin{equation}
%    \begin{aligned}
%        \nabla_{x_t}p_t(x_t|y) 
%        &=  \sbra{-\fs{1}{h(t)}I + \fs{ \alpha^2(t)}{h(t)}AA^\top - \fs{\alpha^2(t)}{\sigma^2 + h(t)\dabs{g_{A}}^2} g_{A} g_{A}^\top }x_t +  \alpha(t) A \mu + \fs{\alpha(t)\rbra{y-h(t)g_{A}^\top A \mu }}{\sigma^2 + h(t)\dabs{g_{A}}^2} \cdot g_A,
 %   \end{aligned}
%\end{equation}


%$\texttt{G}_{loss}$ is
%\begin{equation}
 %     \texttt{G}_{loss} = - \fs{\alpha^2(t)}{\sigma^2 + h(t)\dabs{g_{A}}^2} g_{A} g_{A}^\top x_t + \fs{\alpha(t)\rbra{y-h(t)g_{A}^\top A \mu }}{\sigma^2 + h(t)\dabs{g_{A}}^2} \cdot g_A,
%\end{equation}
%where $g_A = AA^\top g$. Therefore, we get $\texttt{G}_{loss} \in \operatorname{Span}(A)$.


\begin{proof}
We expand the derivative in $\texttt{G}_{loss}$ as
\begin{align*}
\texttt{G}_{loss}(x_t, t) = 2 \beta(t) (y - g^\top \hat{\EE}[x_0 | x_t]) \left(\nabla_{x_t} \hat{\EE}[x_0 | x_t]\right) g.
\end{align*}
Substituting $s_\theta(x_t, t) = \nabla \log p_t(x_t)$ into $\hat{\EE}[x_0 | x_t]$ yields $\hat{\EE}[x_0 | x_t] = \frac{1}{\alpha(t)}(x_t + h(t) \nabla \log p_t(x_t))$. Via the score decomposition under linear subspace data in \citet[Lemma 1]{chen2023score}, we have
\begin{align*}
\nabla \log p_t(x_t) = A \nabla \log p_t^{\sf LD}(A^\top x_t) - \frac{1}{h(t)} \left(I_D - AA^\top \right) x_t,
\end{align*}
where $p_t^{\sf LD}$ denotes the diffused latent distribution, i.e., $p_t^{\sf LD}(u') = \int \phi_t(u'|u_0) p_u(u_0) \dif u_0$. Recall that $\phi_t$ is the Gaussian transition kernel of the forward process and $p_u$ is the density of latent variable $u_0$ in Assumption~\ref{asmp:subspace_data}.

To ease the derivation, we denote $m(u) = \nabla \log p_t^{\sf LD}(u) + \frac{1}{h(t)}u$. It then holds that
\begin{align*}
\hat{\EE}[x_0 | x_t] & = \frac{1}{\alpha(t)} \left(x_t + h(t) \left[Am(A^\top x_t) - \frac{1}{h(t)}x_t\right]\right) \\
& = \frac{h(t)}{\alpha(t)}A m(A^\top x_t).
\end{align*}
As a consequence, we can verify that
\begin{align*}
\nabla_{x_t} \hat{\EE}[x_0 | x_t] = \frac{h(t)}{\alpha(t)} A \left[\nabla m(A^\top x_t)\right] A^\top,
\end{align*}
where $\nabla m(A^\top x_t) = \nabla_u m(u) \in \RR^{d \times d}$. Plugging the last display into $\texttt{G}_{loss}$, we conclude that 
\begin{align*}
\texttt{G}_{loss}(x_t, t) & = 2 \beta(t) (y - g^\top \hat{\EE}[x_0 | x_t]) \left(\nabla_{x_t} \hat{\EE}[x_0 | x_t]\right) g \\
& = \ell_t \cdot g'
\end{align*}
for $\ell_t = 2 \beta(t) (y - g^\top \hat{\EE}[x_0 | x_t])$ and $g' = \left(\nabla_{x_t} \hat{\EE}[x_0 | x_t]\right) g = \frac{h(t)}{\alpha(t)} A \left[\nabla m(A^\top x_t)\right] A^\top g \in {\rm Span}(A)$. 
When $X=AU$ with $U \sim \cN \rbra{\mu, I_d}$, the score function is 
\begin{equation*}
    \nabla \log p_t(x_t) = \rbra{\fs{1}{h(t)}-1} AA^\top x_t - \fs{1}{h(t)} x_t + \alpha(t) A \mu.
\end{equation*}
The correspond look-ahead expectation is
\begin{equation*}
    \EE[x_0|x_t] = \alpha(t)AA^\top x_t + h(t) A \mu.
\end{equation*}
Therefore, it is straightforward that
\begin{equation*}
    \nabla_{x_t} {\EE}[x_0 | x_t]  = \alpha(t) AA^\top,
\end{equation*}
reproducing the projection operator. The proof is complete.
\end{proof}

%Under Assumption \ref{asmp:subspace_data} that data follows $x_0 = Au$, according to \citep{chen2023score}, the groundtruth score is
%\begin{equation}
%    \nabla_{x_t} \log p_t(x_t) = A  \nabla \log p_t^{\text{L}}(A^\top x_t)-\fs{1}{h(t)} \rbra{I_D - AA^\top} x_t,
%\end{equation}
%where 
%\begin{equation*}\label{equ:desity pu}
%    p_t^{\text{L}}(u) = \int \phi_t(u'|u)p_u(u) \dif u,
%\end{equation*}
%with $p_u$ the density for $u$ and with $\phi_t(·|u) $ being the Gaussian density function of $\cN\rbra{\alpha(t)u, h(t)I_d}$.

%Thus, let $ m_1(u) = h(t) \nabla \log p_t^{\text{L}}(u) + u $,
%\begin{equation}
%\begin{aligned}
%    \EE[x_0\mid x_t] &= \fs{1}{\alpha(t)}\rbra{x_t + h(t) \nabla_{x_t} \log p_t(x_t)} \\
%    &= \fs{1}{\alpha(t)}A \rbra{ h(t)   \nabla \log p_t^{\text{L}}(A^\top x_t  ) + A^\top x_t    } \\
%    & = A m_1(A^\top x_t).
%\end{aligned}
%\end{equation}

%Therefore,
%\begin{equation*}
 %   \nabla_{x_t}\rbra{y - g^\top \EE[x_0|x_t]}^2  \propto \nabla_{x_t} \rbra{g^\top \EE[x_0|x_t]}.
%\end{equation*}
%\begin{equation*}
%   \nabla_{x_t} \rbra{g^\top \EE[x_0|x_t]} = \frac{\partial \EE[x_0|x_t]}{\partial x_t} \cdot g = A \frac{\partial m_1(A^\top x_t)}{\partial A^\top x_t} A^\top  g.
%\end{equation*}



==> neurips/appdicies/sde.tex <==
\section{Generation by Backward SDE} \label{append:prof sde solution}

%\paragraph{Variance Control for Generated Data}
%The variance of generated samples $\{z_k\}$ directly influences their diversity.  \cref{alg:main} provides an additional feature for controlling the sample variance, by multiplying the pre-trained score function with a positive scalar $\gamma_k$. Thus $\gamma_k \cdot  s_{\theta}(x_t, t) + \texttt{G} (x_t,  t)$ is used for sampling in the backward process. $\gamma_k$ controls the variance by Lemma \ref{lmm:backward process solution}.

%\paragraph{Solution of Backward SDE}
The following Lemma \ref{lmm:posterior distribution} characterizes the solution of backward SDE to which the score \eqref{equ:score with variance and guidance} is fed, the generated samples are steered by the gradient guidance $\texttt{G}_{loss}$. Note that the tuning parameter $\beta(t)$ needs to be chosen. The following lemma is derived from the perspective of conditional score to get a specified value of $\beta(t)$.

%Note that the tuning parameter
%$\beta(t)$ in \eqref{def:gradient_guidance+} is specified as
%\begin{equation}\label{equ:beta w. subspace}
%    \beta(t) = \fs{\alpha^2(t)/2}{\alpha^2(t) \sigma^2 + h(t)\dabs{ \nabla_{x_t}\rbra{g^\top \hat{\EE}[x_0|x_t]}^2}}.
%\end{equation}

%\paragraph{Choice of $\beta(t)$.} In theoretical analysis, the specification of $\beta(t)$ comes from conditional score functions of data $X = AU$, $A \in \RR^{D \times d}, U \sim \cN \rbra{\mu, I_d}$, $Y\mid X \sim \cN \rbra{g^\top X, \sigma^2}$. The score of marginal distribution $\nabla \log p_t(x_t) $ is
%\begin{equation*}
%\nabla \log p_t(x_t) = -\fs{1}{h(t)}\rbra{I_D - \alpha^2(t) A A^\top}x_t + \alpha(t) A \mu.
%\end{equation*}
%The conditional score $\nabla \log p_t(x_t \mid y)$ is
%\begin{equation*}
 %   \begin{aligned}
 %       \nabla \log p_t(x_t \mid y) &= -\fs{1}{h(t)}\rbra{I_D - \alpha^2(t) A A^\top}x_t + \alpha(t) A \mu \\
 %       &= \fs{ \alpha(t)}{ \sigma^2   + h(t)\dabs{A^\top g}^2}AA^\top g \sbra{ - \alpha(t) g^\top AA^\top x_t  + y - h(t) g^\top A \mu    }. \\
  %      %& = -  \fs{ \alpha^2(t)}{ \sigma^2   + h(t)\dabs{A^\top g}^2}AA^\top g g^\top AA^\top x_t + \fs{\alpha(t)y}{ \sigma^2 + h(t)\dabs{A^\top g}^2}AA^\top g \\&- \fs{\alpha(t) h(t)}{ \sigma^2  + h(t)\dabs{A^\top g}^2} AA^\top gg^\top A \mu.
 %   \end{aligned}
%\end{equation*}
%When selecting $\beta(t)$ as
%\begin{equation*}\label{equ:beta w. subspace groundtruth}
%    \beta(t) = \fs{\alpha^2(t)/2}{\alpha^2(t) \sigma^2 + h(t)\dabs{ \nabla_{x_t}\rbra{g^\top {\EE}[x_0|x_t]}^2}},
%\end{equation*}
%with ${\EE}[x_0|x_t] = \alpha(t) AA^\top x_t + h(t) A \mu $, it holds
%\begin{equation*}
%    \nabla \log p_t(x_t \mid y) =   \nabla \log p_t(x_t) - \beta(t) \cdot \nabla_{x_t} \rbra{y - g^\top {\EE}[x_0|x_t] }^2 =  \nabla \log p_t(x_t) + \texttt{G}_{loss}(x_t,t).
%\end{equation*}
%In other words, if we designate $\beta(t)$ as \eqref{equ:beta w. subspace groundtruth} and the pre-trained score equals with the unconditional score, then the ground truth of the conditional score equals the pre-trained score plus the designed guidance term $\texttt{G}_{loss}(x_t,t)$. Consequently, we opt for beta to be \eqref{equ:beta w. subspace}.


\begin{lemma}\label{lmm:choose beta}
    If the pre-trained score is $s_{\theta}(x_t,t) = -\rbra{\alpha^2(t) \Sigma + h(t) I_D }^{-1}\rbra{x_t - \alpha(t) \mu }$, and $\beta(t)$ is specified as
    \begin{equation}\label{equ:beta w. sigma}
        \beta(t) = \fs{1}{2} \sbra{\sigma^2 + g^\top \rbra{\Sigma^{-1} + \fs{\alpha^2(t)}{h(t)} I_D }^{-1} g     }^{-1},
    \end{equation}
    it holds that
    \begin{equation}\label{equ:beta_guidance_condi}
    \begin{aligned}
      & \quad s_{\theta}(x_t,t) +  \texttt{G}_{loss}(x_t,t) \\
      &= - \rbra{\alpha^2(t)\Sigma + h(t)I_D - \fs{\alpha^2(t)}{\sigma^2 + g^\top \Sigma g } \cdot  \Sigma g  g^\top \Sigma  }^{-1}\sbra{x_t - \rbra{ \alpha(t)\mu + \frac{\alpha(t) \rbra{y - g^\top \mu } }{\sigma^2 + g^\top \Sigma g }\cdot \Sigma g } }.
    \end{aligned}
    \end{equation}
\end{lemma}
\begin{proof}
    We first justify the formula of $s_\theta(x_t,t)$ coincides with the score function in the forward process and \eqref{equ:beta_guidance_condi} coincides with the conditional score function. To be specific, suppose $X_0 \sim \cN \rbra{\mu, \Sigma }, Y = g^\top X_0 + \epsilon $ where $\epsilon \sim \cN (0, \sigma^2 I_D)$ is independent with $X_0$. In the forward process, given $X_0 = x_0$, $X_t$ can be written as $\alpha(t) x_0 + Z_t$ for $Z_t \sim \cN(0, h(t)I_D)$ independent of $x_0$. Due to the linear function assumption, we have
\begin{align*}
\begin{bmatrix}
X_t \\
Y
\end{bmatrix}
=
\begin{bmatrix}
\alpha(t)I_D & 0 & I_D \\
g^\top & 1 & 0
\end{bmatrix}
\begin{bmatrix}
x_0 \\
\epsilon \\
Z_t
\end{bmatrix}.
\end{align*}
Observing that the joint distribution of $(x_0, \epsilon, z_t)$ is Gaussian, we deduce
\begin{align*}
\begin{bmatrix}
X_t \\
Y
\end{bmatrix}
\sim \cN\left(
\begin{bmatrix}
\alpha(t) \mu \\
g^\top \mu
\end{bmatrix},
\begin{bmatrix}
\alpha^2(t) \Sigma + h(t) I_D & \alpha(t) \Sigma g \\
\alpha(t)g^\top \Sigma & \sigma^2 + g^\top \Sigma g
\end{bmatrix}\right).
\end{align*}
The conditional distribution $X_t | Y$ can now be obtained as
\begin{align*}
X_t | Y \sim \cN\left(\alpha(t)\mu + \alpha(t) \frac{y - g^\top \mu}{\sigma^2 + g^\top \Sigma g} \Sigma  g, \alpha^2(t) \Sigma + h(t) I_D -  \frac{\alpha^2(t)}{\sigma^2 + g^\top \Sigma g} \Sigma g   g^\top \Sigma \right).
\end{align*}
Thus the conditional score $\nabla \log p_t(x_t\mid y)$ is exactly as \eqref{equ:beta_guidance_condi}. Also, the marginal distribution of $X_t$ can be obtained as
\begin{equation*}
    X_t \sim \cN \rbra{\alpha(t) \mu,  \alpha^2(t) \Sigma + h(t) I_D },
\end{equation*}
and $s_\theta(x_t,t)$ is the score function. Now we need to derive the guidance $\texttt{G}_{loss}$ computed by $s_\theta$ and $\beta(t)$ and show it satisfies \eqref{equ:beta_guidance_condi}. First, we have
\begin{equation*}
    \begin{aligned}
        \hat{\EE}[x_0|x_t] &= \fs{1}{\alpha(t)}\rbra{x_t + h(t) s_\theta(x_t,t)} \\
        &= \alpha(t) \rbra{\alpha^2(t) \Sigma + h(t) I_D }^{-1} \Sigma  x_t + {h(t)}\rbra{\alpha^2(t) \Sigma + h(t) I_D}^{-1} \mu.
    \end{aligned}
\end{equation*}
Therefore, the guidance $\texttt{G}_{loss}$ is derived as
\begin{equation*}
    \begin{aligned}
        \texttt{G}_{loss}(x_t,t) &= 2 \beta(t) \rbra{y - g^\top \hat{\EE}[x_0|x_t]}\cdot \nabla_{x_t} \hat{\EE}[x_0|x_t] \cdot  g \\
        &= 2 \beta(t) \alpha(t) \sbra{y - \alpha(t) g^\top \Sigma\rbra{\alpha^2(t) \Sigma + h(t) I_D }^{-1}   x_t + {h(t)}g^\top \rbra{\alpha^2(t) \Sigma + h(t) I_D}^{-1} \mu} \\
       & \quad  \cdot \rbra{\alpha^2(t) \Sigma + h(t) I_D }^{-1} \Sigma g.
    \end{aligned}
\end{equation*}
Now, we compare the coefficients of $x_t$, $\mu$ and $y$ in $\nabla \log p_t(x_t|y)$ and $s_\theta(x_t,t) +  \texttt{G}_{loss}(x_t,t)$. To show the two coefficients of $y$ are the same, it suffices to prove
\begin{equation}\label{equ:y coeff}
     \rbra{\alpha^2(t)\Sigma + h(t)I_D - \fs{\alpha^2(t)}{\sigma^2 + g^\top \Sigma g } \cdot  \Sigma g  g^\top \Sigma  }^{-1} \cdot \fs{\alpha(t)}{\sigma^2 + g^\top \Sigma g}\Sigma g = 2\beta(t) \alpha(t) \rbra{\alpha^2(t) \Sigma + h(t) I_D }^{-1} \Sigma g.
\end{equation}
\eqref{equ:y coeff} holds equal to
\begin{equation*}
    \begin{aligned}
    & \Leftrightarrow   \fs{1}{\sigma^2 + g^\top \Sigma g} \Sigma g = 2\beta(t) \cdot \sbra{\Sigma g  - 
     \fs{g^\top \Sigma \rbra{\alpha^2(t) \Sigma + h(t) I_D }^{-1} \Sigma g  }{\sigma^2 + g^\top \Sigma g} \cdot \Sigma g } \\
     & \Leftrightarrow 1/(2\beta(t)) = \sigma^2 + g^\top \Sigma g - g^\top \Sigma \rbra{\alpha^2(t) \Sigma + h(t) I_D }^{-1} \Sigma g.
    \end{aligned}
\end{equation*}
According to Woodbury matrix identity, we have
\begin{equation*}
    \begin{aligned}
       \rbra{\Sigma^{-1} + \fs{\alpha^2(t)}{h(t)} I_D }^{-1} = \Sigma -  \Sigma \rbra{\alpha^2(t) \Sigma + h(t) I_D }^{-1} \Sigma.
    \end{aligned}
\end{equation*}
Thus, \eqref{equ:y coeff} holds for $\beta(t)$ defined in \eqref{equ:beta w. sigma}. The coefficients of $x_t$ and $\mu$ can also be proved to be equal similarly.

\end{proof}

\begin{lemma} \label{lmm:posterior distribution}
If the pre-trained score is $s_\theta (x_t,t)   $ and $\beta(t)$ is assigned as \eqref{equ:beta w. sigma}, substituting the score function with $s_\theta (x_t,t) + \texttt{G}_{loss}(x_t, t) $ in the backward SDE \eqref{eq:backward} yields, when $T \to \infty$,
\begin{equation*}
    X_{T}^{\leftarrow} \sim  \cN\left(\alpha(t)\mu + \alpha(t) \frac{y - g^\top \mu}{\sigma^2 + g^\top \Sigma g} \Sigma  g, \alpha^2(t) \Sigma + h(t) I_D -  \frac{\alpha^2(t)}{\sigma^2 + g^\top \Sigma g} \Sigma g   g^\top \Sigma \right).
\end{equation*}
\end{lemma}

\begin{proof}
Consider $X_0 \sim \cN \rbra{\mu, \Sigma}, Y=g^\top X_0 + \epsilon $ where $\epsilon \sim \cN \rbra{0, \sigma^2 I_D}$. Let $X_0$ be the initialization of the forward process. Denote $p_t(x_t \mid y)$ as the density of $X_t \mid Y$. According to Lemma~\ref{lmm:choose beta} and its proof, we get $ s_\theta (x_t,t) + \texttt{G}_{loss}(x_t, t) = \nabla \log p_t(x_t\mid y) $. Thus, the backward SDE turns out to be
\begin{equation}\label{equ:backward catch condi score}
    \diff \bXb_t = \left[\frac{1}{2} \bXb_t + \nabla \log p_{T-t}(\bXb_t\mid y)\right] \diff t + \diff \overline{W}_t, \quad \bXb_0 \sim \cN \rbra{0, I_D}.
\end{equation}
Since the initial distribution $p_0(x_0 \mid y)$ of the forward process can also be obtained by \eqref{equ:backward catch condi score} where we replace the initial distribution as $p_T(x_T\mid y)$. According to Girsanov theorem, we get the KL divergence between the terminal distribution $p_{T}^{\leftarrow} $ of \eqref{equ:backward catch condi score} and $p_0(x_0 \mid y)$.
\begin{equation*}
    \text{KL}\rbra{p_0 \mid p_{T}^{\leftarrow}  } = - \EE_{p_0} \sbra{\log \rbra{\frac{p_T}{\varphi}}},
\end{equation*}
where $p_0, p_T$ are short hands for $p_0(x_0 \mid y) $ and 
$p_T(x_T\mid y)$, and $\varphi (\cdot)$ is the density for the standard normal distribution $\cN \rbra{0, I_D}$. Since in the forward process, $p_T \to \varphi$ when $T \to \infty $, we have $\text{KL}\rbra{p_0 \mid p_{T}^{\leftarrow}  } \to 0 $ when $T \to \infty$. Thus, the proof is completed.
\end{proof}



\begin{lemma} \label{lmm:backward process solution}
Given the score 
\begin{equation*}
    s(x_t, t) = -\fs{1}{h(t)}\rbra{I - \alpha^2(t) VV^\top} x_t + \alpha(t) V \mu,
\end{equation*}    
with $V^\top V = I_d$, for $\gamma > 1/2$,  define the guided score $s(x_t, y , t)$ as \eqref{equ:score with variance and guidance} with $\texttt{G}= \texttt{G}_{loss} $, i.e.,
\begin{equation*}
    s(x_t, y , t)  = \gamma \cdot s(x_t, t) - \fs{\alpha^2(t)/2}{\alpha^2(t) \sigma^2 + h(t)\dabs{ \nabla_{x_t}\rbra{g^\top \hat{\EE}[x_0|x_t]}^2}} \nabla_{x_t} \rbra{y - g^\top \hat{\EE}[x_0|x_t]}^2.
\end{equation*}
When $s(x_t, y , t)$ is applied to the backward SDEs: 
\begin{equation*}
    \dif X_{t}^{\leftarrow} = \sbra{\fs{1}{2} X_{t}^{ \leftarrow} + \tilde{s}\rbra{X_{t}^{y, \leftarrow}, y, T - t }} \dif t + \dif \overline{W}_t,
\end{equation*}
for $T = \infty$, the generated distribution $X_\infty^{\leftarrow}$ satisfies
\textbf{(i)}
\begin{align*}
    \EE X_\infty^{\leftarrow} &=V \mu + \sbra{c_1\rbra{\gamma, V^\top g} y  + c_2\rbra{\gamma , V^\top g} g^\top  V \mu} \cdot VV^\top g, \label{equ:sample mean}\\ 
    \text{trace}\rbra{\VV X_\infty^{\leftarrow}} &\leq \fs{d}{2\gamma -1},
\end{align*}
where
\begin{align*}
    c_1(\gamma,g') &:=\int_0^\infty \fs{\sigma^2 e^{-\gamma s}}{\rbra{\sigma^2 + \rbra{1-e^{-s}}\dabs{g'}^2}^2} \dif s,\\
    c_2(\gamma,g) &:= \int_0^\infty - \fs{\gamma e^{-\gamma s}\rbra{1-e^{-s}}}{\sigma^2 + \rbra{1-e^{-s}}\dabs{V^\top g}^2} - \fs{\sigma^2 e^{-\gamma s}\rbra{1-e^{-s}}}{\rbra{\sigma^2 + \rbra{1-e^{-s}}\dabs{g'}^2}^2}  \dif s.
\end{align*}
\textbf{(ii)}
$$X_{\infty}^{\leftarrow}   \in \operatorname{Span}(V).$$
\end{lemma}



\begin{proof}
When the pre-trained score is 
\begin{equation*}
    s(x_t, t) = -\fs{1}{h(t)}\rbra{I - \alpha^2(t) VV^\top} x_t + \alpha(t) V \mu,
\end{equation*}
the gradient guided score is
\begin{equation*}
    \begin{aligned}
        s(x_t, y , t) & = \gamma \cdot s(x_t, t) - \beta(t) \nabla_{x_t} \rbra{y - g^\top \hat{\EE}[x_0|x_t]}^2\\
        &=  \sbra{-\fs{\gamma}{h(t)}I + \fs{\gamma \alpha^2(t)}{h(t)}V V^\top - \fs{\alpha^2(t)}{\sigma^2 + h(t)\dabs{g_{V}}^2} g_{V} g_{V}^\top }x_t \\
        &\,\, + \gamma \alpha(t) V \mu + \fs{\alpha(t)\rbra{y-h(t)g_{V}^\top V \mu }}{\sigma^2 + h(t)\dabs{g_{V}}^2} \cdot g_V,
    \end{aligned}
\end{equation*}
where $g_V = VV^\top g$ is the projection of gradient $g$ in the subspace spanned by the columns of $V$. Plug in the score in the backward SDEs:
\begin{equation}\label{equ:backSDE}
    \dif X_t = \sbra{\fs{1}{2}X_t + s(X_t, y , T - t)}\dif t + \dif \overline{W}_t.
\end{equation}
We denote the coefficients of the SDEs as follows.
\begin{align}
    C(t) & := \rbra{\fs{1}{2} - \fs{\gamma}{h(T - t)} }I  + \fs{\gamma \alpha^2(T-t)}{h(T-t)}V V^\top - \fs{\alpha^2(T-t)}{\sigma^2 + h(T-t)\dabs{g_{V}}^2} g_{V} g_{V}^\top, \label{equ:sde matrix}\\
    a(t) &:=  \gamma \alpha(T-t) V \mu + \fs{\alpha(T-t)\rbra{y-h(T-t)g_{V}^\top V \mu }}{\sigma^2 + h(T-t)\dabs{g_{V}}^2} \cdot g_V. \label{equ:sde const}
\end{align}
Therefore, the backward SDE is
\begin{equation*}
    \dif X_t = \rbra{C(t)X_t + a(t)}\dif t + \dif \overline{W}_t.
\end{equation*}
We further define
\begin{equation*}
    B(t) := \exp \rbra{-\int_{0}^t C(s) \dif s }.
\end{equation*}
According to It\^{o}'s Formula, it holds
\begin{equation*}
    \dif {B(t) X_t} = B(t) a(t) \dif t + B(t)  \dif \overline{W}_t.
\end{equation*}
Integrating both sides, we derive
\begin{equation*}
    B(t)X_t - X_0 = \int_0^t B(s) a(s) \dif s + \int_0^t B(s)  \dif \overline{W}_s.
\end{equation*}
Therefore, the solution is
\begin{equation*}
    X_t = B^{-1}(t) X_0 +  \int_0^t B^{-1}(t) B(s) a(s) \dif s + \int_0^t B^{-1}(t) B(s)  \dif \overline{W}_s.
\end{equation*}
Since $X_0 \sim \cN (0, I_D)$, $X_t$ follows Gaussian with
\begin{align*}
    \EE X_t &= \int_0^t B^{-1}(t) B(s) a(s) \dif s , \\
    \VV (X_T) &= B^{-2}(t)+ \int_0^t B^{-2}(t) B^{2}(s)  \dif s .
\end{align*}
Thus, it suffices to calculate $B(t)$. We get
\begin{equation*}
\begin{aligned}
    \int_{0}^t C(s) \dif s &= \sbra{\fs{t}{2}  - \gamma \rbra{t+ \log \fs{1-e^{-T}}{1-e^{-T+t}}}}I + \gamma \log \rbra{\fs{1-e^{-T}}{1-e^{-T+t}}} VV^\top \\
    & - \log \rbra{\fs{\sigma^2 + \rbra{1-e^{-T}}\dabs{g_V}^2}{\sigma^2 + \rbra{1-e^{-T+t}}\dabs{g_V}^2}} \cdot \fs{g_V g_V^\top}{\dabs{g_V}^2}.
\end{aligned}
\end{equation*}
Therefore, it holds
\begin{equation*}
    \begin{aligned}
        B(t) &= \exp \left(  \sbra{ \rbra{\gamma - \fs{1}{2}}t+  \gamma {\log \fs{1-e^{-T}}{1-e^{-T+t}}}}I - \gamma \log \rbra{\fs{1-e^{-T}}{1-e^{-T+t}}} VV^\top  \right. \\
         & \left.  +   \log \rbra{\fs{\sigma^2 + \rbra{1-e^{-T}}\dabs{g_V}^2}{\sigma^2 + \rbra{1-e^{-T+t}}\dabs{g_V}^2}} \cdot \fs{g_V g_V^\top}{\dabs{g_V}^2}   \right). \\
    \end{aligned}
\end{equation*}
We have
\begin{equation*}
    \begin{aligned}
       & \quad B^{-1}(t) B(s) \\
       &= \exp \left(  \sbra{ \rbra{\gamma - \fs{1}{2}}(s-t)+  \gamma {\log \fs{1-e^{-T+t}}{1-e^{-T+s}}}}I + \gamma \log \rbra{\fs{1-e^{-T+s}}{1-e^{-T+t}}} VV^\top \right. \\
       & \quad \quad  \left. +\log \rbra{\fs{\sigma^2 + \rbra{1-e^{-T+t}}\dabs{g_V}^2}{\sigma^2 + \rbra{1-e^{-T+s}}\dabs{g_V}^2}} \cdot \fs{g_V g_V^\top}{\dabs{g_V}^2}   \right)  \\
       & =e^{\rbra{\gamma - 1/2}(s-t)} \rbra{\fs{1-e^{-T+t}}{1-e^{-T+s}}}^{\gamma} \cdot \sbra{I + \rbra{\rbra{\fs{1-e^{-T+s}}{1-e^{-T+t}}}^{\gamma} -1} VV^\top } \\
       &\quad \cdot \sbra{I + \fs{{e^{-T+s}-e^{-T+t}}}{\sigma^2 + \rbra{1-e^{-T+s}}\dabs{g_V}^2} \cdot g_V g_V^\top }.
    \end{aligned}
\end{equation*} 
And it holds
\begin{equation*}
    \begin{aligned}
        &\quad  B^{-1}(t) B(s) a(s) \\
        &= e^{\rbra{\gamma - 1/2}(s-t)-(T-s)/2}\left[ \gamma V \mu + \fs{\sigma^2 + \rbra{1-e^{-T+t}}\dabs{g_V}^2}{\rbra{\sigma^2 + \rbra{1-e^{-T+s}}\dabs{g_V}^2}^2}\cdot y g_V \right. \\
         &\quad \left. + \rbra{\fs{\gamma\rbra{e^{-T+s}-e^{-T+t}}}{\sigma^2 + \rbra{1-e^{-T+s}}\dabs{g_V}^2}- \fs{\rbra{1-e^{-T+s}}\rbra{\sigma^2 + \rbra{1-e^{-T+t}}\dabs{g_V}^2}}{\rbra{\sigma^2 + \rbra{1-e^{-T+s}}\dabs{g_V}^2}^2}  } g_V^\top V \mu \cdot g_V \right].
    \end{aligned}
\end{equation*}
Therefore, if setting $t = T$, it holds
\begin{equation*}
    \begin{aligned}
        \int_{0}^T  B^{-1}(T) B(s) a(s) \dif s &= \int_0^T e^{-\gamma s}\left[ \gamma V \mu + \fs{\sigma^2}{\rbra{\sigma^2 + \rbra{1-e^{-s}}\dabs{g_V}^2}^2}\cdot y g_V \right. \\
         &\quad \left. - \rbra{\fs{\gamma\rbra{1-e^{-s}}}{\sigma^2 + \rbra{1-e^{-s}}\dabs{g_V}^2} + \fs{\sigma^2\rbra{1-e^{-s}}}{\rbra{\sigma^2 + \rbra{1-e^{-s}}\dabs{g_V}^2}^2}  } g_V^\top V \mu \cdot g_V \right] \dif s.
    \end{aligned}
\end{equation*}
Then, the mean of $X_T$ is
\begin{equation*}
    \begin{aligned}
        \EE X_T = \rbra{1-e^{-\gamma T}}V \mu + \sbra{c_1(T,\gamma) y  + c_2(T,\gamma) g_V^\top V \mu} \cdot g_V,
    \end{aligned}
\end{equation*}
where
\begin{align*}
    c_1(T,\gamma) &=\int_0^T \fs{\sigma^2 e^{-\gamma s}}{\rbra{\sigma^2 + \rbra{1-e^{-s}}\dabs{g_V}^2}^2} \dif s,\\
    c_2(T,\gamma) &= \int_0^T - \fs{\gamma e^{-\gamma s}\rbra{1-e^{-s}}}{\sigma^2 + \rbra{1-e^{-s}}\dabs{g_V}^2} - \fs{\sigma^2 e^{-\gamma s}\rbra{1-e^{-s}}}{\rbra{\sigma^2 + \rbra{1-e^{-s}}\dabs{g_V}^2}^2}  \dif s.
\end{align*}
Next, we consider the variance of $X_T$. We have
\begin{equation*}
    \begin{aligned}
        & \quad B^{-2}(t) B^{2}(s) \\
       &= \exp \left(  \sbra{ \rbra{2\gamma - 1}(s-t)+  2\gamma {\log \fs{1-e^{-T+t}}{1-e^{-T+s}}}}I + 2\gamma \log \rbra{\fs{1-e^{-T+s}}{1-e^{-T+t}}} VV^\top \right. \\
       &\quad \quad \left. +   2\log \rbra{\fs{\sigma^2 + \rbra{1-e^{-T+t}}\dabs{g_V}^2}{\sigma^2 + \rbra{1-e^{-T+s}}\dabs{g_V}^2}} \cdot \fs{g_V g_V^\top}{\dabs{g_V}^2}   \right)  \\
       & =e^{\rbra{2\gamma - 1}(s-t)} \rbra{\fs{1-e^{-T+t}}{1-e^{-T+s}}}^{2\gamma} \cdot \sbra{I + \rbra{\rbra{\fs{1-e^{-T+s}}{1-e^{-T+t}}}^{2\gamma} -1} VV^\top } \\
       & \quad \cdot \sbra{I + \rbra{\rbra{\fs{\sigma^2 + \rbra{1-e^{-T+t}}\dabs{g_V}^2}{\sigma^2 + \rbra{1-e^{-T+s}}\dabs{g_V}^2}}^2-1} \cdot \fs{g_V g_V^\top}{\dabs{g_V}^2} } \\
       &= e^{\rbra{2\gamma - 1}(s-t)}\rbra{\fs{1-e^{-T+t}}{1-e^{-T+s}}}^{2\gamma} \rbra{I-VV^\top} + e^{\rbra{2\gamma - 1}(s-t)} VV^\top \\
       &\quad + e^{\rbra{2\gamma - 1}(s-t)} \rbra{\rbra{\fs{\sigma^2 + \rbra{1-e^{-T+t}}\dabs{g_V}^2}{\sigma^2 + \rbra{1-e^{-T+s}}\dabs{g_V}^2}}^2-1} \cdot \fs{g_V g_V^\top}{\dabs{g_V}^2}.
    \end{aligned}
\end{equation*}
Therefore, we get
\begin{equation*}
    \begin{aligned}
        B^{-2}(T) B^{2}(s) &= e^{\rbra{2\gamma - 1}(s-T)} VV^\top + e^{\rbra{2\gamma - 1}(s-T)} \rbra{\rbra{\fs{\sigma^2 }{\sigma^2 + \rbra{1-e^{-T+s}}\dabs{g_V}^2}}^2-1} \cdot \fs{g_V g_V^\top}{\dabs{g_V}^2} .
    \end{aligned}
\end{equation*}
And the trace is
\begin{equation*}
    \begin{aligned}
        \text{trace}\rbra{B^{-2}(T) B^{2}(s)} &= e^{\rbra{2\gamma - 1}(s-T)} \cdot d + e^{\rbra{2\gamma - 1}(s-T)} \rbra{\rbra{\fs{\sigma^2 }{\sigma^2 + \rbra{1-e^{-T+s}}\dabs{g_V}^2}}^2-1} \\
        & \leq e^{\rbra{2\gamma - 1}(s-T)} \cdot d.
    \end{aligned}
\end{equation*}
Thus, we get
\begin{equation*}
    \text{trace}\rbra{\int_0^T B^{-2}(T) B^{2}(s) \dif s} \leq \fs{1- e^{-(2\gamma-1)T}}{2 \gamma -1} \cdot d.
\end{equation*}
To compute the variance, we derive
\begin{equation*}
\begin{aligned}
      B^{-2}(t) &= \exp \left(  \sbra{ \rbra{1-2\gamma}t-2 \gamma {\log \fs{1-e^{-T}}{1-e^{-T+t}}}}I + 2\gamma \log \rbra{\fs{1-e^{-T}}{1-e^{-T+t}}} VV^\top \right.\\
      &\quad \quad \left. -2   \log \rbra{\fs{\sigma^2 + \rbra{1-e^{-T}}\dabs{g_V}^2}{\sigma^2 + \rbra{1-e^{-T+t}}\dabs{g_V}^2}} \cdot \fs{g_V g_V^\top}{\dabs{g_V}^2}   \right)  \\
      &= e^{-(2\gamma-1)t}\rbra{\fs{1-e^{-T+t}}{1-e^{-T}} }^{2\gamma}\cdot \sbra{I + \rbra{\rbra{\fs{1-e^{-T}}{1-e^{-T+t}}}^{2\gamma} -1} VV^\top }  \\
      &\quad \cdot \sbra{I + \rbra{\rbra{\fs{\sigma^2 + \rbra{1-e^{-T+t}}\dabs{g_V}^2}{\sigma^2 + \rbra{1-e^{-T}}\dabs{g_V}^2}}^2-1} \cdot \fs{g_V g_V^\top}{\dabs{g_V}^2} } \\
      &= e^{-(2\gamma-1)t}\cdot \sbra{\rbra{\fs{1-e^{-T+t}}{1-e^{-T}} }^{2\gamma}\rbra{I-VV^\top} + VV^\top } \\
      &\quad  \cdot \sbra{I + \rbra{\rbra{\fs{\sigma^2 + \rbra{1-e^{-T+t}}\dabs{g_V}^2}{\sigma^2 + \rbra{1-e^{-T}}\dabs{g_V}^2}}^2-1} \cdot \fs{g_V g_V^\top}{\dabs{g_V}^2} }. \\
    \end{aligned}
\end{equation*}
Thus, it holds
\begin{equation*}
    \begin{aligned}
        {B^{-2} (T)} = e^{-(2\gamma-1)T}\cdot VV^\top  \cdot \sbra{I + \rbra{\rbra{\fs{\sigma^2 + \rbra{1-e^{-T+t}}\dabs{g_V}^2}{\sigma^2 + \rbra{1-e^{-T}}\dabs{g_V}^2}}^2-1} \cdot \fs{g_V g_V^\top}{\dabs{g_V}^2} } \leq e^{-(2\gamma-1)T}\cdot d.
    \end{aligned}
\end{equation*}
Therefore, we have
\begin{equation*}
    \begin{aligned}
        \text{trace}\rbra{B^{-2} (T)}
    \end{aligned}
\end{equation*}
Thus, we get
\begin{equation*}
   \text{trace}\rbra{\VV X_T} =  \text{trace}\rbra{B^{-2} (T) + \int_0^T B^{-2}(T) B^{2}(s) \dif s} \leq \fs{1- e^{-(2\gamma-1)T}}{2 \gamma -1} \cdot d + e^{-(2\gamma-1)T}\cdot d.
\end{equation*}
If taking the limit, it holds,
\begin{equation*}
    \lim_{T \to \infty } \text{trace}\rbra{\VV X_T} \leq \fs{d}{2\gamma
     -1}.
\end{equation*}
As for \textbf{(ii)}, let $X_t = X_{t,\parallel} + X_{t,\perp}$ where $X_{t,\parallel} \in \operatorname{Span}(V)$ and $X_{t,\perp} \perp \operatorname{Span}(V)$. Then, according to \eqref{equ:backSDE},\eqref{equ:sde matrix} and \eqref{equ:sde const}, the dynamic of $X_{t,\perp}$ is
\begin{equation*}
    \dif X_{t,\perp} = \rbra{\fs{1}{2} - \fs{\gamma}{h(T - t)} }X_{t,\perp}\dif t + (I_D - VV^\top) \dif \overline{W}_t.
\end{equation*}
The variance of $X_{t,\perp}$ is
\begin{equation*}
    \begin{aligned}
       e^{(1-2\gamma)t}\rbra{\fs{1-e^{-T+t}}{1-e^{-T}}}^2 +  \int_0^t e^{(2\gamma -1)(s-t)} \cdot \rbra{\fs{1-e^{-T+t}}{1-e^{-T+s}}}^2 \dif s.
    \end{aligned}
\end{equation*}
Thus, $\VV (X_{T,\perp})=0$. We get $X_{\infty}^{\leftarrow} \in \operatorname{Span}(V)$. 



    
\end{proof}















==> neurips/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}




\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The introduction (\cref{sec:intro}) includes a paragraph ``Scope and Contribution", together with the abstract, clearly reflecting the paper's contributions and scope.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss the limitations in \cref{sec:discussion}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All the theoretical results \cref{lmm:guidance=cond w.o.subspace}, \cref{thm:faith_grad_guidance}, \cref{thm:subspace fully linear} and \cref{thm:w. update w. subspace} provide the full set of assumptions, and the correspond proofs are in \cref{prf:lmm:guidance=cond w.o.subspace}, \cref{prof:faith_grad_guidance}, \cref{pf:subspace fully linear} and \cref{sec:proof of opt theorem update}, respectively.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The main information of the experiments are described in \cref{sec:experiment}, and the details are provided in \cref{sec:experiment details}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The codebase will be released once acceptance is granted.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The experimental details are provided in \cref{sec:experiment details}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The experiments that support the main claims of the paper provide error bars, as shown in \cref{fig:compare_two_G}, \cref{fig:convergence_simulation} and \cref{fig:image_result}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All information on the computer resources is included in \cref{sec:experiment details}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer:\answerYes{}
\item[] Justification: The research adheres to all guidelines and principles outlined in the NeurIPS Code of Ethics, including considerations for fairness, accountability, and transparency. Ethical practices were maintained throughout the study, ensuring compliance with all applicable standards.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss the social impacts of this paper in \cref{sec:discussion}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper poses no such risks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer:  \answerYes{}
\item[] Justification: All creators and original owners of assets used in this paper are properly credited. The licenses and terms of use are explicitly mentioned and respected according to their respective guidelines.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We will release our code and models along with detailed documentation.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing or research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

